Testing Business Cycle Theories: Evidence from the Great Recession

Empirical business cycle studies using cross-country data usually cannot achieve causal relationships while within-country studies mostly focus on the bust period. We provide the first causal investigation into the boom period of the 1999-2010 U.S. cross-metropolitan business cycle. Using a novel research design, we show that credit expansion in private-label mortgages causes a differentially stronger boom (2000-2006) and bust (2007-2010) cycle in the house-related industries in the high net-export-growth areas. Most importantly, our unique research design enables us to perform the most comprehensive tests on theories (hypotheses) regarding the business cycle. We show that the following theories (hypotheses) cannot explain the cause of the 1999-2010 U.S. business cycle: the speculative euphoria hypothesis, the real business cycle theory, the collateral-driven credit cycle theory, the business uncertainty theory, and the extrapolative expectation theory.

==> App_DataDetails.tex <==
%------------------------------------------------------------
%------------------------------------------------------------


%------------------------------------------------------------
\subsection{Appendix for Data Details}\label{subsec:App_Data}


%------------------------------------------------------------
%------------------------------------------------------------
\subsubsection{HMDA Mortgage Data Processing Procedures at ZIP level}
In this section, I illustrate the processing details regarding the mortgage data at the ZIP code level. I will describe the processes of crosswalking from census tracts to ZIP codes, retaining data in the 1990-2000-unchanged ZIP codes, linking ZIP codes to primary counties and metropolitan areas, mortgage data requirement at the ZIP level, and grouping ZIP codes into income groups within metropolitan areas. 

\paragraph{Crosswalk from Census Tracts to ZIP Codes} 
First, I use the 712 or 800 consistent counties across time to filter HMDA data, depending on the period of interest. Second, HMDA mortgage data uses various versions of census tracts across time. 1981-1991, 1992-2002, and 2003-2009 HMDA datasets use 1980, 1990, and 2000 versions of the census tract, respectively. From the Missouri Census Data Center \footnote{Missouri Census Data Center's website is here: \url{https://mcdc.missouri.edu/applications/geocorr.html}}, I obtain the crosswalk file that links 1980 census tracts to 1990 ZIP codes, that links 1990 census tracts to 1990 ZIP codes, and that links 2000 census tracts to 2000 ZIP codes. I use population weight in the crosswalk since multiple census tracts can match multiple ZIP codes. I use 1992-1999 as the prior period for comparison because I intend to retain a reasonably large number of ZIP codes in a balanced panel for comparison. To prevent within-ZIP code changes from contaminating my analysis, I only keep ZIP codes that are mostly covered by HMDA reporting. Specifically, I keep ZIP codes with populations crosswalked from the HMDA mortgage data that are equal to or above 90\% of the ZIP total population. The deleted ZIP codes are mostly the ZIP codes on the boundary of metropolitan areas, since HMDA mainly covers metropolitan areas. 

ZIP codes are reasonably large areas within metropolitan areas. One ZIP code typically contains several census blocks, which are designed to provide more statistical uniformity with an average of 4,000 plus population. In the 1992-2009 mortgage panel data of 9995 ZIP codes, ZIP codes contain a population size of 4237, 12610, and 26023 at 25\%, 50\%, and 75\%, respectively. \footnote{For more information comparing census tracts and ZIP codes, see \url{https://proximityone.com/tracts_zips.htm}.}



\paragraph{Retaining Data in the 1990-2000-unchanged ZIP codes}
According to \cite{bailey2023national}, ZIP code geographic boundary can change in relationship to population growth and decline across time. For example, their detailed work based on The Postal Bulletin by the U.S. Postal Office shows that 3015 changes happened between 1990 and 2000. This number of changes is not small given 29,401 distinct ZIP codes were in operation at the beginning of 1990 (by the crosswalk file from the Missouri Census Data Center described above). Typical changes include merge, split, and boundary alteration. These changes can result in measurement error (matching observations to the wrong unites) or missing data (due to an observation reporting a ZIP code that did not in operation at the beginning of the sample period). 

To avoid the potential measurement error and missing data, I get a list of 1990-2000-unchanged ZIP codes by following steps. First, from the Missouri Census Data Center, I get the crosswalk file from 1990 ZIP codes to 1990 counties with population weights. Second, I delete any ZIP codes that may experience change during 1990-2000 from the 1990 ZIP codes list. Specifically, I delete ZIP codes that appear in the following variables in the following files by \cite{bailey2023national}: (1) variable ``oldzipcode" or ``newzipcode" in file ``ZIP\_Code\_Changes\_1990-2000\_Documentation.xls" and (2) ``zipcode" in file ``ZIP\_xwalk\_90-00.dta". Out of the 29,401 ZIP codes in the year 1990, 26,577 ZIP codes did not experience any change. Third, I match these ZIP codes to ZIP codes in the crosswalk file from 2000 ZIP codes to 2000 counties with population weights. I retain only matched ZIP codes. The above three steps result in 
26,058 1990-2000-unchanged ZIP codes. 

\paragraph{Link ZIP codes to Their Primary Counties and Metropolitan Areas}
One ZIP code can be linked to multiple counties (metropolitan areas) when it exists on the border. For each match zip code, I only keep its primary matched county that contains the most population in the zip code. From the Missouri Census Data Center, I get the crosswalk file that links 2000 ZIP codes to 2000 counties. I retain counties in the 2003 version of metropolitan areas in U.S. mainland (excluding Hawaii and Alaska).\footnote{Metropolitan areas definition (CBSA code) of 2003 can be found here: \url{https://www2.census.gov/programs\%2Dsurveys/metro\%2Dmicro/geographies/reference\%2Dfiles/2003/historical\%2Ddelineation\%2Dfiles/030606omb\%2Dnecta\%2Dcnecta.xls}.} 


The above steps result in 13,513 1990-2000-unchanged ZIP codes that are matched to primary counties in the metropolitan areas (2003 version CBSA code) in the U.S. mainland. I use these ZIP codes to filter HMDA ZIP-level data. 

 
\paragraph{Mortgage Data Requirement at the ZIP Level}\label{subsec:MortgageData_ZIP}
I require each ZIP code to have mortgage data in all years of analysis (1992-2009 for figure and 1999-2009 for regression analysis). I also require each ZIP code must have nonzero value for government-sponsored enterprise mortgages, private-label mortgages (non-jumbo), and mortgages retained on the balance sheet of financial institutions in the initial year (either 1992 or 1999). This requirement make sure that each ZIP code has starting value and non-missing growth rate in the main analysis.\footnote{This step also excludes ZIP codes with a tiny population.} The resulting 1992-2009 (1999-2009) mortgage panel data contains 9,995 (10,785) ZIP codes from 693 (782) counties.


\paragraph{Group ZIP codes Within Metropolitan Areas}
To conduct analysis in Section (\ref{subsec:ModelNewPrediction_Empirical})) for the model-based new predictions, I need to sum mortgage data in ZIP codes into half-, tertile-, quartile-, and quintile-income groups within metropolitan areas. To make sure each metropolitan statistic area (MSA) contains enough ZIP codes for calculation, I require that each MSA contains at least three ZIP codes for the calculation of half- and tertile-income groups and at least five ZIP codes for the calculation of quartile- and quintile-income groups. Since ZIP codes are reasonably large areas (with a population size of 4237 and 26023 at 25\% and 75\% in the 1992-2009 mortgage panel data), I believe three (five) ZIP codes are a good minimum number for the calculation.  



%------------------------------------------------------------
%------------------------------------------------------------
\subsubsection{House Price Data at ZIP level}
The annual house price index at the ZIP level based on repeat sales comes from the Federal Housing Financing Agency.\footnote{The data website of the Federal Housing Financing Agency is here: \url{https://www.fhfa.gov/DataTools/Downloads/Pages/House-Price-Index-Datasets.aspx#qexe}.} This database has reasonably good coverage of the ZIP codes of US metropolitan areas in and after 1992 (11,556 ZIP codes in 1992) but a little bit less coverage than the HMDA mortgage data.

\paragraph{Merge House Price and Mortgage Data at ZIP Level}
For both figure and regression analysis regarding house prices, I require that the ZIP codes are covered by both house price data and mortgage data refined in Section \ref{subsec:MortgageData_ZIP}. The merged data set contains fewer ZIP codes compared to mortgage data since house price data covers fewer ZIP codes. Second, I require that each zip code contains both data 1992-2009 (1999-2009) for figure (regression analysis). 


\paragraph{Interpolating House Units}
I collect the number of house units at the ZIP level from Decennial Census Summary Files in 1900 (File 3B), 2000 (File 1), and 2010 (File 1). Since Census data are collected as of March in 1990, 2000, and 2010, I treat the number of house units as the one at the end of last year (1989, 1999, and 2009, respectively). I interpolate the number of house units from 1990 to 2008 by a linear function. Then, I merge house unit data with the prices-mortgage merged data. For the final data, I require that each MSA contains at least three ZIP codes for the calculation of half- and tertile-income groups and at least five ZIP codes for the calculation of quartile- and quintile-income groups. 

Due to data availability of house prices and house units, the final data contains fewer ZIP codes than the mortgage data. The 1992-2009 half- (quintile-) income group data for figure contains 6,083 (5,942) ZIP codes from 244 (204) metropolitan areas. The 1999-2009 half- (quintile-) income group data for regression analysis contains 8,517 (8,427) ZIP codes from 293 (268) metropolitan areas.


\comment{
Lastly, I use the number of house units as weights to aggregate house prices across zip code groups within metropolitan areas. 
}

==> Empirical.DoubleDifference.tex <==
%------------------------------------------------------------
%------------------------------------------------------------
%\clearpage
%------------------------------------------------------------
%------------------------------------------------------------
\section{Empirical Results: ``Double Difference"}


==> Figure/fig_ConstEmpShrB92_92To11.tex <==

%------------------------------------------------------------
% figure 1: fig_ConstEmpShrB92_92To11

\begin{figure}[h!] 
    \centering
    \includegraphics[width=16cm, height=12cm]{Figure/12_Figure_9_BEACty_ConstEmpShrB92_QuintD92t06NEPV91_HMDA90On_612Cty_92To11}
    \caption{\textbf{Construction Employment Share (92-11) in Metro Areas, Top vs. Bottom Quintile of Net Export Growth (92 to 06)} \smallskip \newline 
    {\footnotesize This figure displays the time series of weighted average construction employment share in the working-age population for top and bottom quintile groups of Metropolitan Areas (MSAs) from 1992 to 2011. For the entire period, the quintile groups are sorted by net export growth (1992 to 2006) at the metropolitan level (CBSA code 2003 version). The sample includes 285 metropolitan areas (612 counties) that are consistently covered by the Bureau of Economic Analysis (BEA) Employment data between 1992 and 2011. These 612 out of HMDA consistent 712 counties have non-missing and non-zero construction employment observations from 1992 to 2011. The bottom quintile group comprises 55 metros (87 counties), and the top quintile group comprises 54 metros (93 counties) throughout the entire period. The construction employment share is weighted by the county-level working-age population (age between 15 and 64) within each group in each year. Throughout the entire period, the time series of weighted-average construction employment shares of each group are divided by their 1992 values, ensuring that both groups start at a value of 1 in 1992. The red line represents the top quintile group, while the blue line represents the bottom quintile group.
    } %end of small font
    } % end of caption
    \label{fig_ConstEmpShrB92_92To11}
    % note that \label is given after \caption.
\end{figure} 



==> Figure/fig_SelfEmpShrB92_92To11.tex <==

%------------------------------------------------------------
% figure 1: fig_SelfEmpShrB92_92To11

\begin{figure}[h!] 
    \centering
    \includegraphics[width=16cm, height=12cm]{Figure/12_Figure_3_BEACty_ProprietEmpShrB92_QuintD92t06NEPV91_HMDA90On_687Cty_92To11.png}
    \caption{\textbf{Self-Employment Share (92-11) in Metro Areas, Top vs. Bottom Quintile of Net Export Growth (92 to 06)} \smallskip \newline 
    {\footnotesize This figure displays the time series of weighted average self-employment share in the working-age population for top and bottom quintile groups of Metropolitan Areas (MSAs) from 1992 to 2011. For the entire period, the quintile groups are sorted by net export growth (1992 to 2006) at the metropolitan level (CBSA code 2003 version). The sample includes 299 metropolitan areas (687 counties) that are consistently covered by the Bureau of Economic Analysis (BEA) Employment sample between 1992 and 2011. These 687 out of HMDA consistent 712 counties have non-missing self-employment data from 1992 to 2011. The bottom quintile group comprises 60 metros (101 counties), and the top quintile group comprises 59 metros (110 counties) throughout the entire period. The self-employment share is weighted by the county-level working-age population (age between 15 and 64) within each group in each year. Throughout the entire period, the time series of the weighted average self-employment share of each group is divided by their 1992 values, ensuring that both groups start at a value of 1 in 1992. The red line represents the top quintile group, while the blue line represents the bottom quintile group.
    } %end of small font
    } % end of caption
    \label{fig_SelfEmpShrB92_92To11}
    % note that \label is given after \caption.
\end{figure} 



==> Figure/fig_TotEmpShrB92_92To11.tex <==

%------------------------------------------------------------
% figure 1: fig_TotEmpShrB92_92To11
% the following content is not correct. If I need to show EmpShrB92, I need to revise the entire content 

\begin{figure}[h!] 
    \centering
    \includegraphics[width=16cm, height=12cm]{Figure/7_Graph_1_BEACty_TotEmpShr_QuintD92t06NEPV91_HMDA92On_687Cty_92To11.png}
    \caption{\textbf{Total Employment Share (92-11) in Metro Areas, Top vs. Bottom Quintile of Net Export Growth (91 to 07)} \smallskip \newline 
    {\footnotesize This figure displays the time series of weighted average total employment share in the working-age population for top and bottom quintile groups of Metropolitan Areas (MSAs) from 1992 to 2011. For the entire period, the quintile groups are sorted by net export growth (1991 to 2007) at the metropolitan level (CBSA code 2003 version). The sample includes 299 metropolitan areas (687 counties) that are consistently covered by the Bureau of Economic Analysis (BEA) Employment sample between 1992 and 2011. These 687 out of HMDA consistent 712 counties have non-missing employment data from 1992 to 2011 from Bureau of Economics Analylis in the U.S. Department of Commerce. The bottom quintile group comprises 60 metros (91 counties), and the top quintile group comprises 59 metros (104 counties) throughout the entire period. The total employment share is weighted by working-age population (age between 15 and 64) within each group in each year. Throughout the entire period, the time series of the weighted average total employment share of each group is divided by their 1992 values, ensuring that both groups start at a value of 1 in 1992. The red line represents the top quintile group, while the blue line represents the bottom quintile group.
    } %end of small font
    } % end of caption
    \label{fig_TotEmpShrB92_92To11}
    % note that \label is given after \caption.
\end{figure} 



==> Table_Purch/table_BEA.ConstEmpShr.D00t06vsD07t10.PLMNJ.D99t05.2SLS.tex <==
%-----------------------------------------------------------------------
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% table_BEA.ConstEmpShr.D00t06vsD07t10.PLMNJ.D99t05.2SLS
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\noindent 

\begin{table}[h!]
\centering
\caption{
\textbf{2SLS Stacked Regression of Construction Employment Growth in Boom (00-06) and Bust (07-10) Periods on PLMNJ Growth (99-05)} \smallskip \newline
{\scriptsize
This table reports 2SLS regression $\triangle_{00,06} \& \triangle_{07,10} ConstEmpShr_{c} = \beta_{00,06} * \triangle_{99,05} Ln(PLMNJ_{c}) \times Dum_{00,06} + \beta_{07,10} * \triangle_{99,05} Ln(PLMNJ_{c}) \times Dum_{07,10} + \gamma_{00,06}* \bm{Controls_{c}} \times Dum_{00,06} + \gamma_{07,10}* \bm{Controls_{c}} \times Dum_{07,10} + \epsilon_{period, c}$. The left-hand-side dependent variable $\triangle_{00,06} \& \triangle_{07,10} ConstEmpShr_{c}$ is the change of the construction employment share in working-age population at county $c$ 00-06 and 07-10. To reduce the impact of outliers, dependent variable is winsorized at 1\% and 99\% levels in each period. The key independent variable $\triangle_{99,05} Ln(PLMNJ_{c})$ is the growth rate of the dollar amount (07USD) of private-label mortgages (non-jumbo) at county $c$ 99-05. $Controls_{c}$ indicates control variables at county $c$ in the period start year 1999. We use the gravity model-based instrumental variable $\triangle_{99,05}\text{givNetExp}_{m}$ as the IV for $\triangle_{99,05}Ln(PLMNJ_{c})$. Regression is weighted by the natural logarithm of housing units in 1999.  For the first-stage F-test of two non-stacked samples, we report Kleibergen-Paap (2006) robust (clustered) statistics and Montiel Olea-Pflueger (2013) efficient statistics. Standard errors are clustered at the CBSA level. ***, **, and * indicate significance at the 1\%, 5\%, and 10\% levels, respectively.
\smallskip
} % end of small font size
} % end of caption
\label{table_BEA.ConstEmpShr.D00t06vsD07t10.PLMNJ.D99t05.2SLS}

\vspace{-2mm}

\resizebox{0.55\columnwidth}{!}{%
\begin{tabular}{l*{4}{c}}
\toprule
\textbf{TSLS estimates}            &\multicolumn{4}{c}{Construction Employment Growth (00-06 and 07-10, An)} \\
            \cmidrule{2-5} 
            &\multicolumn{1}{c}{(1)}&\multicolumn{1}{c}{(2)}&\multicolumn{1}{c}{(3)}&\multicolumn{1}{c}{(4)}\\
            
\midrule
PLMNJ Growth (07USD, 99-05, An) x Dum00t06&    0.015***&    0.015***&    0.013** &    0.015** \\
               &  (0.005)   &  (0.005)   &  (0.006)   &  (0.006)   \\
\addlinespace
PLMNJ Growth (07USD, 99-05, An) x Dum07t10&   -0.022***&   -0.019** &   -0.018*  &   -0.022** \\
               &  (0.008)   &  (0.008)   &  (0.010)   &  (0.011)   \\
\addlinespace
Dum00t06       &   -0.002*  &   -0.012***&   -0.014***&    0.000   \\
               &  (0.001)   &  (0.004)   &  (0.005)   &  (0.008)   \\
\addlinespace
Dum07t10       &   -0.000   &    0.032***&    0.026***&   -0.000   \\
               &  (0.001)   &  (0.008)   &  (0.010)   &  (0.017)   \\
\addlinespace
Ln(Num of HH, 99) x Dum00t06&            &   -0.000** &   -0.003***&   -0.003***\\
               &            &  (0.000)   &  (0.001)   &  (0.001)   \\
\addlinespace
Ln(Num of HH, 99) x Dum07t10&            &   -0.000   &   -0.001   &   -0.000   \\
               &            &  (0.000)   &  (0.002)   &  (0.002)   \\
\addlinespace
Ln(HH Income, 99) x Dum00t06&            &    0.001***&    0.001***&   -0.000   \\
               &            &  (0.000)   &  (0.000)   &  (0.001)   \\
\addlinespace
Ln(HH Income, 99) x Dum07t10&            &   -0.003***&   -0.002*  &    0.000   \\
               &            &  (0.001)   &  (0.001)   &  (0.002)   \\
\addlinespace
Ratio of Labor Force (1999) x Dum00t06&            &   -0.005***&   -0.003   &   -0.003   \\
               &            &  (0.002)   &  (0.002)   &  (0.002)   \\
\addlinespace
Ratio of Labor Force (1999) x Dum07t10&            &   -0.000   &   -0.006   &   -0.007   \\
               &            &  (0.004)   &  (0.004)   &  (0.004)   \\
\addlinespace
Ln(Num of HU, 99) x Dum00t06&            &            &    0.003***&    0.003***\\
               &            &            &  (0.001)   &  (0.001)   \\
\addlinespace
Ln(Num of HU, 99) x Dum07t10&            &            &    0.000   &   -0.000   \\
               &            &            &  (0.002)   &  (0.002)   \\
\addlinespace
Housing supply elasticity x Dum00t06&            &            &    0.000   &    0.000   \\
               &            &            &  (0.000)   &  (0.000)   \\
\addlinespace
Housing supply elasticity x Dum07t10&            &            &    0.000   &   -0.000   \\
               &            &            &  (0.000)   &  (0.000)   \\
\addlinespace
House Vacancy Rate (1999) x Dum00t06&            &            &    0.000   &   -0.001   \\
               &            &            &  (0.003)   &  (0.003)   \\
\addlinespace
House Vacancy Rate (1999) x Dum07t10&            &            &   -0.010   &   -0.007   \\
               &            &            &  (0.007)   &  (0.006)   \\
\addlinespace
Ratio of Renters (1999) x Dum00t06&            &            &   -0.003*  &   -0.004** \\
               &            &            &  (0.002)   &  (0.002)   \\
\addlinespace
Ratio of Renters (1999) x Dum07t10&            &            &    0.006** &    0.011***\\
               &            &            &  (0.003)   &  (0.003)   \\
\addlinespace
Ratio of Bachelor Educated (1999) x Dum00t06&            &            &            &    0.004   \\
               &            &            &            &  (0.002)   \\
\addlinespace
Ratio of Bachelor Educated (1999) x Dum07t10&            &            &            &   -0.006   \\
               &            &            &            &  (0.004)   \\
\addlinespace
Ratio of White Race (1999) x Dum00t06&            &            &            &    0.001   \\
               &            &            &            &  (0.001)   \\
\addlinespace
Ratio of White Race (1999) x Dum07t10&            &            &            &    0.001   \\
               &            &            &            &  (0.002)   \\
\addlinespace
Ratio of Immigration (90-00) x Dum00t06&            &            &            &    0.012***\\
               &            &            &            &  (0.004)   \\
\addlinespace
Ratio of Immigration (90-00) x Dum07t10&            &            &            &   -0.021** \\
               &            &            &            &  (0.010)   \\
\midrule
Obs            &     1530   &     1530   &     1368   &     1368   \\
Cluster SE     &     CBSA   &     CBSA   &     CBSA   &     CBSA   \\
Weight         & Ln(HU99)   & Ln(HU99)   & Ln(HU99)   & Ln(HU99)   \\
KP F-Stat (99-05, non-stack sample)       &    20.97   &    19.44   &    12.87   &    10.48   \\
MOP F-Stat (99-05, non-stack sample)  &    20.00   &    18.89   &    12.85   &    10.47   \\
CoefEqual\_Chi2  &   10.192   &    8.385   &    4.154   &    5.548   \\
CoefEqual\_PValue &    0.001   &    0.004   &    0.042   &    0.019   \\
\bottomrule

\end{tabular}

} % end of resize box

\end{table}

==> Table_Purch/table_BEA.Farm.D00t06vsD07t10.PLMNJ.2SLS.tex <==
%-----------------------------------------------------------------------
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% table_BEA.Farm.D00t06vsD07t10.PLMNJ.2SLS
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\noindent 

\begin{table}[h!]
\centering
\caption{
\textbf{2SLS Stacked Regression of Farm Employment Growth in Boom (00-06) and Bust (07-10) Periods on PLMNJ Growth (99-05)} \smallskip \newline
{\scriptsize
This table reports 2SLS regression $\triangle_{00,06} \& \triangle_{07,10} FarmEmpShr_{c} = \beta_{00,06} * \triangle_{99,05} Ln(PLMNJ_{c}) \times Dum_{00,06} + \beta_{07,10} * \triangle_{99,05} Ln(PLMNJ_{c}) \times Dum_{07,10} + \gamma_{00,06}* \bm{Controls_{c}} \times Dum_{00,06} + \gamma_{07,10}* \bm{Controls_{c}} \times Dum_{07,10} + \epsilon_{period, c}$. The left-hand-side dependent variable $\triangle_{00,06} \& \triangle_{07,10} FarmEmpShr_{c}$ is the change of the Farm employment share in working-age population at county $c$ 00-06 and 07-10. The key independent variable $\triangle_{99,05} Ln(PLMNJ_{c})$ is the growth rate of the dollar amount (07USD) of private-label mortgages (non-jumbo) at county $c$ 99-05. $Controls_{c}$ indicates control variables at county $c$ in the period start year 1999. We use the gravity model-based instrumental variable $\triangle_{99,05}\text{givNetExp}_{m}$ as the IV for $\triangle_{99,05}Ln(PLMNJ_{c})$. Regression is weighted by the natural logarithm of housing units in 1999.  For the first-stage F-test of two non-stacked samples, we report Kleibergen-Paap (2006) robust (clustered) statistics and Montiel Olea-Pflueger (2013) efficient statistics. Standard errors are clustered at the CBSA level. ***, **, and * indicate significance at the 1\%, 5\%, and 10\% levels, respectively.
\smallskip
} % end of small font size
} % end of caption
\label{table_BEA.Farm.D00t06vsD07t10.PLMNJ.2SLS}

\vspace{-2mm}

\resizebox{0.55\columnwidth}{!}{%
\begin{tabular}{l*{4}{c}}
\toprule
\textbf{TSLS estimates}            &\multicolumn{4}{c}{BEA Farm Employment Growth (00-06 and 07-10, An)} \\
            \cmidrule{2-5} 
            &\multicolumn{1}{c}{(1)}&\multicolumn{1}{c}{(2)}&\multicolumn{1}{c}{(3)}&\multicolumn{1}{c}{(4)}\\
            
\midrule
PLMNJ Growth (07USD, 99-05, An) x Dum00t06&   -0.114   &   -0.323   &   -0.313   &   -0.436   \\
               &  (0.243)   &  (0.267)   &  (0.320)   &  (0.301)   \\
\addlinespace
PLMNJ Growth (07USD, 99-05, An) x Dum07t10&    0.131   &    0.094   &    0.118   &    0.129   \\
               &  (0.122)   &  (0.129)   &  (0.165)   &  (0.177)   \\
\addlinespace
Dum00t06       &   -0.053   &   -0.617***&   -0.725***&   -0.489   \\
               &  (0.040)   &  (0.167)   &  (0.208)   &  (0.369)   \\
\addlinespace
Dum07t10       &   -0.039*  &   -0.169** &   -0.233** &   -0.001   \\
               &  (0.021)   &  (0.084)   &  (0.115)   &  (0.246)   \\
\addlinespace
Ln(Num of HH, 99) x Dum00t06&            &    0.039***&   -0.045   &    0.014   \\
               &            &  (0.005)   &  (0.038)   &  (0.042)   \\
\addlinespace
Ln(Num of HH, 99) x Dum07t10&            &    0.006** &   -0.003   &    0.004   \\
               &            &  (0.003)   &  (0.022)   &  (0.024)   \\
\addlinespace
Ln(HH Income, 99) x Dum00t06&            &    0.015   &    0.013   &   -0.003   \\
               &            &  (0.018)   &  (0.021)   &  (0.034)   \\
\addlinespace
Ln(HH Income, 99) x Dum07t10&            &    0.004   &    0.011   &   -0.010   \\
               &            &  (0.009)   &  (0.012)   &  (0.023)   \\
\addlinespace
Ratio of Labor Force (1999) x Dum00t06&            &    0.012   &    0.106   &   -0.008   \\
               &            &  (0.082)   &  (0.098)   &  (0.097)   \\
\addlinespace
Ratio of Labor Force (1999) x Dum07t10&            &    0.032   &    0.037   &    0.018   \\
               &            &  (0.044)   &  (0.051)   &  (0.055)   \\
\addlinespace
Ln(Num of HU, 99) x Dum00t06&            &            &    0.090** &    0.036   \\
               &            &            &  (0.040)   &  (0.043)   \\
\addlinespace
Ln(Num of HU, 99) x Dum07t10&            &            &    0.006   &   -0.002   \\
               &            &            &  (0.021)   &  (0.023)   \\
\addlinespace
Housing supply elasticity x Dum00t06&            &            &    0.001   &   -0.003   \\
               &            &            &  (0.005)   &  (0.005)   \\
\addlinespace
Housing supply elasticity x Dum07t10&            &            &    0.002   &    0.002   \\
               &            &            &  (0.003)   &  (0.003)   \\
\addlinespace
House Vacancy Rate (1999) x Dum00t06&            &            &    0.045   &    0.110   \\
               &            &            &  (0.101)   &  (0.100)   \\
\addlinespace
House Vacancy Rate (1999) x Dum07t10&            &            &    0.005   &    0.001   \\
               &            &            &  (0.072)   &  (0.075)   \\
\addlinespace
Ratio of Renters (1999) x Dum00t06&            &            &   -0.042   &    0.046   \\
               &            &            &  (0.075)   &  (0.065)   \\
\addlinespace
Ratio of Renters (1999) x Dum07t10&            &            &    0.069** &    0.053   \\
               &            &            &  (0.035)   &  (0.049)   \\
\addlinespace
Ratio of Bachelor Educated (1999) x Dum00t06&            &            &            &    0.224** \\
               &            &            &            &  (0.097)   \\
\addlinespace
Ratio of Bachelor Educated (1999) x Dum07t10&            &            &            &    0.083   \\
               &            &            &            &  (0.068)   \\
\addlinespace
Ratio of White Race (1999) x Dum00t06&            &            &            &   -0.067*  \\
               &            &            &            &  (0.040)   \\
\addlinespace
Ratio of White Race (1999) x Dum07t10&            &            &            &   -0.009   \\
               &            &            &            &  (0.024)   \\
\addlinespace
Ratio of Immigration (90-00) x Dum00t06&            &            &            &   -1.313***\\
               &            &            &            &  (0.290)   \\
\addlinespace
Ratio of Immigration (90-00) x Dum07t10&            &            &            &   -0.056   \\
               &            &            &            &  (0.089)   \\

\midrule
Obs            &     1530   &     1530   &     1368   &     1368   \\
Cluster SE     &     CBSA   &     CBSA   &     CBSA   &     CBSA   \\
Weight         & Ln(HU99)   & Ln(HU99)   & Ln(HU99)   & Ln(HU99)   \\
KP F-Stat (99-05, non-stack sample)       &    20.97   &    19.44   &    12.87   &    10.48   \\
MOP F-Stat (99-05, non-stack sample)  &    20.00   &    18.89   &    12.85   &    10.47   \\
CoefEqual\_Chi2  &    0.970   &    2.507   &    1.803   &    3.284   \\
CoefEqual\_PValue  &    0.325   &    0.113   &    0.179   &    0.070   \\
\bottomrule

\end{tabular}

} % end of resize box

\end{table}

==> Table_Purch/table_BEA.Farm.D00t06vsD07t10.PLMNJ.2SLS.wide.tex <==
%-----------------------------------------------------------------------
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% table_BEA.Farm.D00t06vsD07t10.PLMNJ.2SLS.wide
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\noindent 

\begin{table}[h!]
\centering
\caption{
\textbf{2SLS Stacked Regression of Farm Employment Growth in Boom (00-06) and Bust (07-10) Periods on PLMNJ Growth (99-05)} \smallskip \newline
{\scriptsize
This table reports 2SLS regression $\triangle_{00,06} \& \triangle_{07,10} FarmEmpShr_{c} = \beta_{00,06} * \triangle_{99,05} Ln(PLMNJ_{c}) \times Dum_{00,06} + \beta_{07,10} * \triangle_{99,05} Ln(PLMNJ_{c}) \times Dum_{07,10} + \gamma_{00,06}* \bm{Controls_{c}} \times Dum_{00,06} + \gamma_{07,10}* \bm{Controls_{c}} \times Dum_{07,10} + \epsilon_{period, c}$. The left-hand-side dependent variable $\triangle_{00,06} \& \triangle_{07,10} FarmEmpShr_{c}$ is the change of the Farm employment share in working-age population at county $c$ 00-06 and 07-10. The key independent variable $\triangle_{99,05} Ln(PLMNJ_{c})$ is the growth rate of the dollar amount (07USD) of private-label mortgages (non-jumbo) at county $c$ 99-05. $Controls_{c}$ indicates control variables at county $c$ in the period start year 1999. We use the gravity model-based instrumental variable $\triangle_{99,05}\text{givNetExp}_{m}$ as the IV for $\triangle_{99,05}Ln(PLMNJ_{c})$. Regression is weighted by the natural logarithm of housing units in 1999.  For the first-stage F-test of two non-stacked samples, we report Kleibergen-Paap (2006) robust (clustered) statistics and Montiel Olea-Pflueger (2013) efficient statistics. Standard errors are clustered at the CBSA level. ***, **, and * indicate significance at the 1\%, 5\%, and 10\% levels, respectively.
\smallskip
} % end of small font size
} % end of caption
\label{table_BEA.Farm.D00t06vsD07t10.PLMNJ.2SLS.wide}

\vspace{-2mm}

\resizebox{\columnwidth}{!}{%
\begin{tabular}{l*{8}{c}}
\toprule
\textbf{TSLS estimates}            &\multicolumn{8}{c}{Farm Employment Growth (00-06 and 07-10, An)} \\
            \cmidrule{2-9} 
            &\multicolumn{2}{c}{(1)}&\multicolumn{2}{c}{(2)}&\multicolumn{2}{c}{(3)}&\multicolumn{2}{c}{(4)}\\
            
\midrule
PLMNJ Growth (07USD, 99-05, An) x Dum00t06&   -0.114   &  (0.243)&   -0.323   &  (0.267)&   -0.313   &  (0.320)&   -0.436   &  (0.301)\\ 
\addlinespace
PLMNJ Growth (07USD, 99-05, An) x Dum07t10&    0.131   &  (0.122)&    0.094   &  (0.129)&    0.118   &  (0.165)&    0.129   &  (0.177)\\ 
\addlinespace
Dum00t06       &   -0.053   &  (0.040)&   -0.617***&  (0.167)&   -0.725***&  (0.208)&   -0.489   &  (0.369)\\ 
\addlinespace
Dum07t10       &   -0.039*  &  (0.021)&   -0.169** &  (0.084)&   -0.233** &  (0.115)&   -0.001   &  (0.246)\\ 
\addlinespace
Ln(Num of HH, 99) x Dum00t06&            &         &    0.039***&  (0.005)&   -0.045   &  (0.038)&    0.014   &  (0.042)\\ 
\addlinespace
Ln(Num of HH, 99) x Dum07t10&            &         &    0.006** &  (0.003)&   -0.003   &  (0.022)&    0.004   &  (0.024)\\ 
\addlinespace
Ln(HH Income, 99) x Dum00t06&            &         &    0.015   &  (0.018)&    0.013   &  (0.021)&   -0.003   &  (0.034)\\ 
\addlinespace
Ln(HH Income, 99) x Dum07t10&            &         &    0.004   &  (0.009)&    0.011   &  (0.012)&   -0.010   &  (0.023)\\ 
\addlinespace
Ratio of Labor Force (1999) x Dum00t06&            &         &    0.012   &  (0.082)&    0.106   &  (0.098)&   -0.008   &  (0.097)\\ 
\addlinespace
Ratio of Labor Force (1999) x Dum07t10&            &         &    0.032   &  (0.044)&    0.037   &  (0.051)&    0.018   &  (0.055)\\ 
\addlinespace
Ln(Num of HU, 99) x Dum00t06&            &         &            &         &    0.090** &  (0.040)&    0.036   &  (0.043)\\ 
\addlinespace
Ln(Num of HU, 99) x Dum07t10&            &         &            &         &    0.006   &  (0.021)&   -0.002   &  (0.023)\\ 
\addlinespace
Housing supply elasticity x Dum00t06&            &         &            &         &    0.001   &  (0.005)&   -0.003   &  (0.005)\\ 
\addlinespace
Housing supply elasticity x Dum07t10&            &         &            &         &    0.002   &  (0.003)&    0.002   &  (0.003)\\ 
\addlinespace
House Vacancy Rate (1999) x Dum00t06&            &         &            &         &    0.045   &  (0.101)&    0.110   &  (0.100)\\ 
\addlinespace
House Vacancy Rate (1999) x Dum07t10&            &         &            &         &    0.005   &  (0.072)&    0.001   &  (0.075)\\ 
\addlinespace
Ratio of Renters (1999) x Dum00t06&            &         &            &         &   -0.042   &  (0.075)&    0.046   &  (0.065)\\ 
\addlinespace
Ratio of Renters (1999) x Dum07t10&            &         &            &         &    0.069** &  (0.035)&    0.053   &  (0.049)\\ 
\addlinespace
Ratio of Bachelor Educated (1999) x Dum00t06&            &         &            &         &            &         &    0.224** &  (0.097)\\ 
\addlinespace
Ratio of Bachelor Educated (1999) x Dum07t10&            &         &            &         &            &         &    0.083   &  (0.068)\\ 
\addlinespace
Ratio of White Race (1999) x Dum00t06&            &         &            &         &            &         &   -0.067*  &  (0.040)\\ 
\addlinespace
Ratio of White Race (1999) x Dum07t10&            &         &            &         &            &         &   -0.009   &  (0.024)\\ 
\addlinespace
Ratio of Immigration (90-00) x Dum00t06&            &         &            &         &            &         &   -1.313***&  (0.290)\\ 
\addlinespace
Ratio of Immigration (90-00) x Dum07t10&            &         &            &         &            &         &   -0.056   &  (0.089)\\ 
\addlinespace
\midrule
Obs            &     1530   &         &     1530   &         &     1368   &         &     1368   &         \\
Cluster SE     &     CBSA   &         &     CBSA   &         &     CBSA   &         &     CBSA   &         \\
Weight         & Ln(HU99)   &         & Ln(HU99)   &         & Ln(HU99)   &         & Ln(HU99)   &         \\
KP F-Stat (99-05, non-stack sample)      &    20.97   &         &    19.44   &         &    12.87   &         &    10.48   &         \\
MOP F-Stat (99-05, non-stack sample)  &    20.00   &         &    18.89   &         &    12.85   &         &    10.47   &         \\
CoefEqual\_Chi2 &    0.970   &         &    2.507   &         &    1.803   &         &    3.284   &         \\
CoefEqual\_PValue &    0.325   &         &    0.113   &         &    0.179   &         &    0.070   &         \\
\bottomrule

\end{tabular}

} % end of resize box

\end{table}

==> Table_Purch/table_BEA.Manufacture.D00t06vsD07t10.PLMNJ.2SLS.tex <==
%-----------------------------------------------------------------------
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% table_BEA.Manufacture.D00t06vsD07t10.PLMNJ.2SLS
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\noindent 

\begin{table}[h!]
\centering
\caption{
\textbf{2SLS Stacked Regression of Manufacture Employment Growth in Boom (00-06) and Bust (07-10) Periods on PLMNJ Growth (99-05)} \smallskip \newline
{\scriptsize
This table reports 2SLS regression $\triangle_{00,06} \& \triangle_{07,10} ManufactureEmpShr_{c} = \beta_{00,06} * \triangle_{99,05} Ln(PLMNJ_{c}) \times Dum_{00,06} + \beta_{07,10} * \triangle_{99,05} Ln(PLMNJ_{c}) \times Dum_{07,10} + \gamma_{00,06}* \bm{Controls_{c}} \times Dum_{00,06} + \gamma_{07,10}* \bm{Controls_{c}} \times Dum_{07,10} + \epsilon_{period, c}$. The left-hand-side dependent variable $\triangle_{00,06} \& \triangle_{07,10} ManufactureEmpShr_{c}$ is the change of the manufacture employment share in working-age population at county $c$ 00-06 and 07-10. The key independent variable $\triangle_{99,05} Ln(PLMNJ_{c})$ is the growth rate of the dollar amount (07USD) of private-label mortgages (non-jumbo) at county $c$ 99-05. $Controls_{c}$ indicates control variables at county $c$ in the period start year 1999. We use the gravity model-based instrumental variable $\triangle_{99,05}\text{givNetExp}_{m}$ as the IV for $\triangle_{99,05}Ln(PLMNJ_{c})$. Regression is weighted by the natural logarithm of housing units in 1999.  For the first-stage F-test of two non-stacked samples, we report Kleibergen-Paap (2006) robust (clustered) statistics and Montiel Olea-Pflueger (2013) efficient statistics. Standard errors are clustered at the CBSA level. ***, **, and * indicate significance at the 1\%, 5\%, and 10\% levels, respectively.
\smallskip
} % end of small font size
} % end of caption
\label{table_BEA.Manufacture.D00t06vsD07t10.PLMNJ.2SLS}

\vspace{-2mm}

\resizebox{0.55\columnwidth}{!}{%
\begin{tabular}{l*{4}{c}}
\toprule
\textbf{TSLS estimates}            &\multicolumn{4}{c}{BEA Manufacture Employment Growth (00-06 and 07-10, An)} \\
            \cmidrule{2-5} 
            &\multicolumn{1}{c}{(1)}&\multicolumn{1}{c}{(2)}&\multicolumn{1}{c}{(3)}&\multicolumn{1}{c}{(4)}\\
            
\midrule
PLMNJ Growth (07USD, 99-05, An) x Dum00t06&    0.064***&    0.072***&    0.081***&    0.091***\\
               &  (0.024)   &  (0.025)   &  (0.028)   &  (0.029)   \\
\addlinespace
PLMNJ Growth (07USD, 99-05, An) x Dum07t10&    0.062***&    0.064***&    0.070***&    0.077***\\
               &  (0.020)   &  (0.020)   &  (0.025)   &  (0.028)   \\
\addlinespace
Dum00t06       &   -0.015***&    0.008   &   -0.020   &    0.096***\\
               &  (0.004)   &  (0.016)   &  (0.022)   &  (0.036)   \\
\addlinespace
Dum07t10       &   -0.015***&   -0.017   &   -0.045** &    0.062*  \\
               &  (0.003)   &  (0.015)   &  (0.019)   &  (0.032)   \\
\addlinespace
Ln(Num of HH, 99) x Dum00t06&            &   -0.001***&    0.002   &    0.003   \\
               &            &  (0.000)   &  (0.004)   &  (0.004)   \\
\addlinespace
Ln(Num of HH, 99) x Dum07t10&            &   -0.000   &   -0.003   &   -0.000   \\
               &            &  (0.000)   &  (0.004)   &  (0.004)   \\
\addlinespace
Ln(HH Income, 99) x Dum00t06&            &   -0.001   &    0.002   &   -0.008** \\
               &            &  (0.002)   &  (0.002)   &  (0.004)   \\
\addlinespace
Ln(HH Income, 99) x Dum07t10&            &    0.001   &    0.004** &   -0.005*  \\
               &            &  (0.002)   &  (0.002)   &  (0.003)   \\
\addlinespace
Ratio of Labor Force (1999) x Dum00t06&            &   -0.001   &   -0.013   &   -0.017   \\
               &            &  (0.008)   &  (0.010)   &  (0.012)   \\
\addlinespace
Ratio of Labor Force (1999) x Dum07t10&            &   -0.008   &   -0.016*  &   -0.023** \\
               &            &  (0.007)   &  (0.009)   &  (0.010)   \\
\addlinespace
Ln(Num of HU, 99) x Dum00t06&            &            &   -0.004   &   -0.005   \\
               &            &            &  (0.004)   &  (0.004)   \\
\addlinespace
Ln(Num of HU, 99) x Dum07t10&            &            &    0.002   &   -0.001   \\
               &            &            &  (0.004)   &  (0.004)   \\
\addlinespace
Housing supply elasticity x Dum00t06&            &            &    0.001** &    0.001***\\
               &            &            &  (0.000)   &  (0.000)   \\
\addlinespace
Housing supply elasticity x Dum07t10&            &            &    0.001*  &    0.001*  \\
               &            &            &  (0.000)   &  (0.000)   \\
\addlinespace
House Vacancy Rate (1999) x Dum00t06&            &            &   -0.002   &   -0.007   \\
               &            &            &  (0.011)   &  (0.012)   \\
\addlinespace
House Vacancy Rate (1999) x Dum07t10&            &            &   -0.006   &   -0.009   \\
               &            &            &  (0.010)   &  (0.012)   \\
\addlinespace
Ratio of Renters (1999) x Dum00t06&            &            &    0.011** &   -0.003   \\
               &            &            &  (0.006)   &  (0.006)   \\
\addlinespace
Ratio of Renters (1999) x Dum07t10&            &            &    0.012** &    0.003   \\
               &            &            &  (0.005)   &  (0.006)   \\
\addlinespace
Ratio of Bachelor Educated (1999) x Dum00t06&            &            &            &    0.036***\\
               &            &            &            &  (0.011)   \\
\addlinespace
Ratio of Bachelor Educated (1999) x Dum07t10&            &            &            &    0.036***\\
               &            &            &            &  (0.010)   \\
\addlinespace
Ratio of White Race (1999) x Dum00t06&            &            &            &   -0.004   \\
               &            &            &            &  (0.004)   \\
\addlinespace
Ratio of White Race (1999) x Dum07t10&            &            &            &   -0.002   \\
               &            &            &            &  (0.004)   \\
\addlinespace
Ratio of Immigration (90-00) x Dum00t06&            &            &            &    0.019   \\
               &            &            &            &  (0.025)   \\
\addlinespace
Ratio of Immigration (90-00) x Dum07t10&            &            &            &   -0.003   \\
               &            &            &            &  (0.017)   \\
\midrule
Obs            &     1530   &     1530   &     1368   &     1368   \\
Cluster SE     &     CBSA   &     CBSA   &     CBSA   &     CBSA   \\
Weight         & Ln(HU99)   & Ln(HU99)   & Ln(HU99)   & Ln(HU99)   \\
KP F-Stat (99-05, non-stack sample)       &    20.97   &    19.44   &    12.87   &    10.48   \\
MOP F-Stat (99-05, non-stack sample)  &    20.00   &    18.89   &    12.85   &    10.47   \\
CoefEqual\_Chi2  &    0.016   &    0.231   &    0.310   &    0.479   \\
CoefEqual\_PValue  &    0.898   &    0.631   &    0.578   &    0.489   \\
\bottomrule

\end{tabular}

} % end of resize box

\end{table}

==> Table_Purch/table_BEA.Manufacture.D00t06vsD07t10.PLMNJ.2SLS.wide.tex <==
%-----------------------------------------------------------------------
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% table_BEA.Manufacture.D00t06vsD07t10.PLMNJ.2SLS.wide
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\noindent 

\begin{table}[h!]
\centering
\caption{
\textbf{2SLS Stacked Regression of Manufacture Employment Growth in Boom (00-06) and Bust (07-10) Periods on PLMNJ Growth (99-05)} \smallskip \newline
{\scriptsize
This table reports 2SLS regression $\triangle_{00,06} \& \triangle_{07,10} ManufactureEmpShr_{c} = \beta_{00,06} * \triangle_{99,05} Ln(PLMNJ_{c}) \times Dum_{00,06} + \beta_{07,10} * \triangle_{99,05} Ln(PLMNJ_{c}) \times Dum_{07,10} + \gamma_{00,06}* \bm{Controls_{c}} \times Dum_{00,06} + \gamma_{07,10}* \bm{Controls_{c}} \times Dum_{07,10} + \epsilon_{period, c}$. The left-hand-side dependent variable $\triangle_{00,06} \& \triangle_{07,10} ManufactureEmpShr_{c}$ is the change of the manufacture employment share in working-age population at county $c$ 00-06 and 07-10. The key independent variable $\triangle_{99,05} Ln(PLMNJ_{c})$ is the growth rate of the dollar amount (07USD) of private-label mortgages (non-jumbo) at county $c$ 99-05. $Controls_{c}$ indicates control variables at county $c$ in the period start year 1999. We use the gravity model-based instrumental variable $\triangle_{99,05}\text{givNetExp}_{m}$ as the IV for $\triangle_{99,05}Ln(PLMNJ_{c})$. Regression is weighted by the natural logarithm of housing units in 1999.  For the first-stage F-test of two non-stacked samples, we report Kleibergen-Paap (2006) robust (clustered) statistics and Montiel Olea-Pflueger (2013) efficient statistics. Standard errors are clustered at the CBSA level. ***, **, and * indicate significance at the 1\%, 5\%, and 10\% levels, respectively.
\smallskip
} % end of small font size
} % end of caption
\label{table_BEA.Manufacture.D00t06vsD07t10.PLMNJ.2SLS.wide}

\vspace{-2mm}

\resizebox{\columnwidth}{!}{%
\begin{tabular}{l*{8}{c}}
\toprule
\textbf{TSLS estimates}            &\multicolumn{8}{c}{Farm Employment Growth (00-06 and 07-10, An)} \\
            \cmidrule{2-9} 
            &\multicolumn{2}{c}{(1)}&\multicolumn{2}{c}{(2)}&\multicolumn{2}{c}{(3)}&\multicolumn{2}{c}{(4)}\\
            
\midrule
PLMNJ Growth (07USD, 99-05, An) x Dum00t06&    0.064***&  (0.024)&    0.072***&  (0.025)&    0.081***&  (0.028)&    0.091***&  (0.029)\\ \addlinespace
PLMNJ Growth (07USD, 99-05, An) x Dum07t10&    0.062***&  (0.020)&    0.064***&  (0.020)&    0.070***&  (0.025)&    0.077***&  (0.028)\\ \addlinespace
Dum00t06       &   -0.015***&  (0.004)&    0.008   &  (0.016)&   -0.020   &  (0.022)&    0.096***&  (0.036)\\ 
\addlinespace
Dum07t10       &   -0.015***&  (0.003)&   -0.017   &  (0.015)&   -0.045** &  (0.019)&    0.062*  &  (0.032)\\ 
\addlinespace
Ln(Num of HH, 99) x Dum00t06&            &         &   -0.001***&  (0.000)&    0.002   &  (0.004)&    0.003   &  (0.004)\\ 
\addlinespace
Ln(Num of HH, 99) x Dum07t10&            &         &   -0.000   &  (0.000)&   -0.003   &  (0.004)&   -0.000   &  (0.004)\\ 
\addlinespace
Ln(HH Income, 99) x Dum00t06&            &         &   -0.001   &  (0.002)&    0.002   &  (0.002)&   -0.008** &  (0.004)\\ 
\addlinespace
Ln(HH Income, 99) x Dum07t10&            &         &    0.001   &  (0.002)&    0.004** &  (0.002)&   -0.005*  &  (0.003)\\ 
\addlinespace
Ratio of Labor Force (1999) x Dum00t06&            &         &   -0.001   &  (0.008)&   -0.013   &  (0.010)&   -0.017   &  (0.012)\\ 
\addlinespace
Ratio of Labor Force (1999) x Dum07t10&            &         &   -0.008   &  (0.007)&   -0.016*  &  (0.009)&   -0.023** &  (0.010)\\ 
\addlinespace
Ln(Num of HU, 99) x Dum00t06&            &         &            &         &   -0.004   &  (0.004)&   -0.005   &  (0.004)\\ 
\addlinespace
Ln(Num of HU, 99) x Dum07t10&            &         &            &         &    0.002   &  (0.004)&   -0.001   &  (0.004)\\ 
\addlinespace
Housing supply elasticity x Dum00t06&            &         &            &         &    0.001** &  (0.000)&    0.001***&  (0.000)\\ 
\addlinespace
Housing supply elasticity x Dum07t10&            &         &            &         &    0.001*  &  (0.000)&    0.001*  &  (0.000)\\ 
\addlinespace
House Vacancy Rate (1999) x Dum00t06&            &         &            &         &   -0.002   &  (0.011)&   -0.007   &  (0.012)\\ 
\addlinespace
House Vacancy Rate (1999) x Dum07t10&            &         &            &         &   -0.006   &  (0.010)&   -0.009   &  (0.012)\\ 
\addlinespace
Ratio of Renters (1999) x Dum00t06&            &         &            &         &    0.011** &  (0.006)&   -0.003   &  (0.006)\\ 
\addlinespace
Ratio of Renters (1999) x Dum07t10&            &         &            &         &    0.012** &  (0.005)&    0.003   &  (0.006)\\ 
\addlinespace
Ratio of Bachelor Educated (1999) x Dum00t06&            &         &            &         &            &         &    0.036***&  (0.011)\\ 
\addlinespace
Ratio of Bachelor Educated (1999) x Dum07t10&            &         &            &         &            &         &    0.036***&  (0.010)\\ 
\addlinespace
Ratio of White Race (1999) x Dum00t06&            &         &            &         &            &         &   -0.004   &  (0.004)\\  \addlinespace
Ratio of White Race (1999) x Dum07t10&            &         &            &         &            &         &   -0.002   &  (0.004)\\  \addlinespace
Ratio of Immigration (90-00) x Dum00t06&            &         &            &         &            &         &    0.019   &  (0.025)\\  \addlinespace
Ratio of Immigration (90-00) x Dum07t10&            &         &            &         &            &         &   -0.003   &  (0.017)\\  \addlinespace
\midrule
Obs            &     1530   &         &     1530   &         &     1368   &         &     1368   &         \\
Cluster SE     &     CBSA   &         &     CBSA   &         &     CBSA   &         &     CBSA   &         \\
Weight         & Ln(HU99)   &         & Ln(HU99)   &         & Ln(HU99)   &         & Ln(HU99)   &         \\
KP F-Stat (99-05, non-stack sample)      &    20.97   &         &    19.44   &         &    12.87   &         &    10.48   &         \\
MOP F-Stat (99-05, non-stack sample)  &    20.00   &         &    18.89   &         &    12.85   &         &    10.47   &         \\
CoefEqual\_Chi2 &    0.016   &         &    0.231   &         &    0.310   &         &    0.479   &         \\
CoefEqual\_PValue &    0.898   &         &    0.631   &         &    0.578   &         &    0.489   &         \\
\bottomrule

\end{tabular}

} % end of resize box

\end{table}

==> Table_Purch/table_ComConst.D00t06vsD07t10.PLMNJ.2SLS.tex <==
%-----------------------------------------------------------------------
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% table_ComConst.D00t06vsD07t10.PLMNJ.2SLS
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\noindent 

\begin{table}[h!]
\centering
\caption{
\textbf{2SLS Stacked Regression of Commercial Construction Employment Growth in Boom (00-06) and Bust (07-10) Periods on PLMNJ Growth (99-05)} \smallskip \newline
{\scriptsize
This table reports 2SLS regression $\triangle_{00,06} \& \triangle_{07,10} ComConstEmpShr_{c} = \beta_{00,06} * \triangle_{99,05} Ln(PLMNJ_{c}) \times Dum_{00,06} + \beta_{07,10} * \triangle_{99,05} Ln(PLMNJ_{c}) \times Dum_{07,10} + \gamma_{00,06}* \bm{Controls_{c}} \times Dum_{00,06} + \gamma_{07,10}* \bm{Controls_{c}} \times Dum_{07,10} + \epsilon_{period, c}$. The left-hand-side dependent variable $\triangle_{00,06} \& \triangle_{07,10} ComConstEmpShr_{c}$ is the change of the commercial construction employment share in working-age population at county $c$ 00-06 and 07-10. The key independent variable $\triangle_{99,05} Ln(PLMNJ_{c})$ is the growth rate of the dollar amount (07USD) of private-label mortgages (non-jumbo) at county $c$ 99-05. $Controls_{c}$ indicates control variables at county $c$ in the period start year 1999. We use the gravity model-based instrumental variable $\triangle_{99,05}\text{givNetExp}_{m}$ as the IV for $\triangle_{99,05}Ln(PLMNJ_{c})$. Regression is weighted by the natural logarithm of housing units in 1999.  For the first-stage F-test of two non-stacked samples, we report Kleibergen-Paap (2006) robust (clustered) statistics and Montiel Olea-Pflueger (2013) efficient statistics. Standard errors are clustered at the CBSA level. ***, **, and * indicate significance at the 1\%, 5\%, and 10\% levels, respectively.
\smallskip
} % end of small font size
} % end of caption
\label{table_ComConst.D00t06vsD07t10.PLMNJ.2SLS}

\vspace{-2mm}

\resizebox{0.55\columnwidth}{!}{%
\begin{tabular}{l*{4}{c}}
\toprule
\textbf{TSLS estimates}            &\multicolumn{4}{c}{Commercial Construction Employment Growth (00-06 and 07-10, An)} \\
            \cmidrule{2-5} 
            &\multicolumn{1}{c}{(1)}&\multicolumn{1}{c}{(2)}&\multicolumn{1}{c}{(3)}&\multicolumn{1}{c}{(4)}\\
            
\midrule
PLMNJ Growth (99-05, An) x Dum00t06&   -0.079   &   -0.101   &   -0.235   &   -0.223   \\
               &  (0.166)   &  (0.173)   &  (0.217)   &  (0.209)   \\
\addlinespace
PLMNJ Growth (99-05, An) x Dum07t10&    0.007   &    0.049   &    0.017   &   -0.008   \\
               &  (0.120)   &  (0.129)   &  (0.185)   &  (0.188)   \\
\addlinespace
Dum00t06       &    0.014   &   -0.107   &    0.065   &    0.093   \\
               &  (0.027)   &  (0.098)   &  (0.241)   &  (0.378)   \\
\addlinespace
Dum07t10       &   -0.017   &    0.489***&    0.669***&    0.623** \\
               &  (0.020)   &  (0.140)   &  (0.175)   &  (0.283)   \\
\addlinespace
Ln(Num of HH, 99) x Dum00t06&            &    0.003   &    0.078   &    0.071   \\
               &            &  (0.005)   &  (0.097)   &  (0.100)   \\
\addlinespace
Ln(Num of HH, 99) x Dum07t10&            &    0.003   &    0.054*  &    0.054*  \\
               &            &  (0.003)   &  (0.028)   &  (0.031)   \\
\addlinespace
Ln(HH Income, 99) x Dum00t06&            &    0.010   &   -0.013   &   -0.014   \\
               &            &  (0.012)   &  (0.027)   &  (0.039)   \\
\addlinespace
Ln(HH Income, 99) x Dum07t10&            &   -0.054***&   -0.065***&   -0.059** \\
               &            &  (0.015)   &  (0.018)   &  (0.028)   \\
\addlinespace
Ratio of Labor Force (1999) x Dum00t06&            &   -0.027   &   -0.002   &    0.010   \\
               &            &  (0.035)   &  (0.045)   &  (0.051)   \\
\addlinespace
Ratio of Labor Force (1999) x Dum07t10&            &    0.050   &   -0.015   &   -0.012   \\
               &            &  (0.064)   &  (0.065)   &  (0.069)   \\
\addlinespace
Ln(Num of HU, 99) x Dum00t06&            &            &   -0.066   &   -0.060   \\
               &            &            &  (0.088)   &  (0.091)   \\
\addlinespace
Ln(Num of HU, 99) x Dum07t10&            &            &   -0.052*  &   -0.051*  \\
               &            &            &  (0.027)   &  (0.030)   \\
\addlinespace
Housing supply elasticity x Dum00t06&            &            &   -0.000   &    0.000   \\
               &            &            &  (0.002)   &  (0.002)   \\
\addlinespace
Housing supply elasticity x Dum07t10&            &            &    0.001   &   -0.000   \\
               &            &            &  (0.004)   &  (0.004)   \\
\addlinespace
House Vacancy Rate (1999) x Dum00t06&            &            &    0.239   &    0.230   \\
               &            &            &  (0.153)   &  (0.150)   \\
\addlinespace
House Vacancy Rate (1999) x Dum07t10&            &            &   -0.032   &   -0.028   \\
               &            &            &  (0.083)   &  (0.085)   \\
\addlinespace
Ratio of Renters (1999) x Dum00t06&            &            &   -0.123   &   -0.141   \\
               &            &            &  (0.092)   &  (0.103)   \\
\addlinespace
Ratio of Renters (1999) x Dum07t10&            &            &   -0.017   &   -0.016   \\
               &            &            &  (0.038)   &  (0.049)   \\
\addlinespace
Ratio of Bachelor Educated (1999) x Dum00t06&            &            &            &   -0.005   \\
               &            &            &            &  (0.064)   \\
\addlinespace
Ratio of Bachelor Educated (1999) x Dum07t10&            &            &            &   -0.002   \\
               &            &            &            &  (0.076)   \\
\addlinespace
Ratio of White Race (1999) x Dum00t06&            &            &            &   -0.005   \\
               &            &            &            &  (0.016)   \\
\addlinespace
Ratio of White Race (1999) x Dum07t10&            &            &            &   -0.026   \\
               &            &            &            &  (0.025)   \\
\addlinespace
Ratio of Immigration (90-00) x Dum00t06&            &            &            &    0.110   \\
               &            &            &            &  (0.090)   \\
\addlinespace
Ratio of Immigration (90-00) x Dum07t10&            &            &            &   -0.147   \\
               &            &            &            &  (0.115)   \\
\midrule
Obs            &     1548   &     1548   &     1367   &     1367   \\
Cluster SE     &     CBSA   &     CBSA   &     CBSA   &     CBSA   \\
Weight         & Ln(HU99)   & Ln(HU99)   & Ln(HU99)   & Ln(HU99)   \\
KP F-Stat (99-05, non-stack sample)       &    23.12   &    21.09   &    13.79   &    11.63   \\
MOP F-Stat (99-05, non-stack sample)  &    22.05   &    20.35   &    13.82   &    11.66   \\
CoefEqual\_Chi2  &    0.134   &    0.363   &    0.606   &    0.473   \\
CoefEqual\_PValue &    0.714   &    0.547   &    0.436   &    0.492   \\
\bottomrule

\end{tabular}

} % end of resize box

\end{table}

==> Table_Purch/table_ComConst.D00t06vsD07t10.PLMNJ.2SLS.wide.tex <==
%-----------------------------------------------------------------------
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% table_ComConst.D00t06vsD07t10.PLMNJ.2SLS.wide
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\noindent 

\begin{table}[h!]
\centering
\caption{
\textbf{2SLS Stacked Regression of Commercial Construction Employment Growth in Boom (00-06) and Bust (07-10) Periods on PLMNJ Growth (99-05)} \smallskip \newline
{\scriptsize
This table reports 2SLS regression $\triangle_{00,06} \& \triangle_{07,10} ComConstEmpShr_{c} = \beta_{00,06} * \triangle_{99,05} Ln(PLMNJ_{c}) \times Dum_{00,06} + \beta_{07,10} * \triangle_{99,05} Ln(PLMNJ_{c}) \times Dum_{07,10} + \gamma_{00,06}* \bm{Controls_{c}} \times Dum_{00,06} + \gamma_{07,10}* \bm{Controls_{c}} \times Dum_{07,10} + \epsilon_{period, c}$. The left-hand-side dependent variable $\triangle_{00,06} \& \triangle_{07,10} ComConstEmpShr_{c}$ is the change of the commercial construction employment share in working-age population at county $c$ 00-06 and 07-10. The key independent variable $\triangle_{99,05} Ln(PLMNJ_{c})$ is the growth rate of the dollar amount (07USD) of private-label mortgages (non-jumbo) at county $c$ 99-05. $Controls_{c}$ indicates control variables at county $c$ in the period start year 1999. We use the gravity model-based instrumental variable $\triangle_{99,05}\text{givNetExp}_{m}$ as the IV for $\triangle_{99,05}Ln(PLMNJ_{c})$. Regression is weighted by the natural logarithm of housing units in 1999.  For the first-stage F-test of two non-stacked samples, we report Kleibergen-Paap (2006) robust (clustered) statistics and Montiel Olea-Pflueger (2013) efficient statistics. Standard errors are clustered at the CBSA level. ***, **, and * indicate significance at the 1\%, 5\%, and 10\% levels, respectively.
\smallskip
} % end of small font size
} % end of caption
\label{table_ComConst.D00t06vsD07t10.PLMNJ.2SLS.wide}

\vspace{-2mm}

\resizebox{\columnwidth}{!}{%
\begin{tabular}{l*{8}{c}}
\toprule
\textbf{TSLS estimates}            &\multicolumn{8}{c}{Commercial Construction Employment Growth (00-06 and 07-10, An)} \\
            \cmidrule{2-9} 
            &\multicolumn{2}{c}{(1)}&\multicolumn{2}{c}{(2)}&\multicolumn{2}{c}{(3)}&\multicolumn{2}{c}{(4)}\\
            
\midrule
PLMNJ Growth (99-05, An) x Dum00t06&   -0.079   &  (0.166)&   -0.101   &  (0.173)&   -0.235   &  (0.217)&   -0.223   &  (0.209)\\ 
\addlinespace
PLMNJ Growth (99-05, An) x Dum07t10&    0.007   &  (0.120)&    0.049   &  (0.129)&    0.017   &  (0.185)&   -0.008   &  (0.188)\\ 
\addlinespace
Dum00t06       &    0.014   &  (0.027)&   -0.107   &  (0.098)&    0.065   &  (0.241)&    0.093   &  (0.378)\\ 
\addlinespace
Dum07t10       &   -0.017   &  (0.020)&    0.489***&  (0.140)&    0.669***&  (0.175)&    0.623** &  (0.283)\\ 
\addlinespace
Ln(Num of HH, 99) x Dum00t06&            &         &    0.003   &  (0.005)&    0.078   &  (0.097)&    0.071   &  (0.100)\\ 
\addlinespace
Ln(Num of HH, 99) x Dum07t10&            &         &    0.003   &  (0.003)&    0.054*  &  (0.028)&    0.054*  &  (0.031)\\ 
\addlinespace
Ln(HH Income, 99) x Dum00t06&            &         &    0.010   &  (0.012)&   -0.013   &  (0.027)&   -0.014   &  (0.039)\\ 
\addlinespace
Ln(HH Income, 99) x Dum07t10&            &         &   -0.054***&  (0.015)&   -0.065***&  (0.018)&   -0.059** &  (0.028)\\ 
\addlinespace
Ratio of Labor Force (1999) x Dum00t06&            &         &   -0.027   &  (0.035)&   -0.002   &  (0.045)&    0.010   &  (0.051)\\ 
\addlinespace
Ratio of Labor Force (1999) x Dum07t10&            &         &    0.050   &  (0.064)&   -0.015   &  (0.065)&   -0.012   &  (0.069)\\ 
\addlinespace
Ln(Num of HU, 99) x Dum00t06&            &         &            &         &   -0.066   &  (0.088)&   -0.060   &  (0.091)\\ 
\addlinespace
Ln(Num of HU, 99) x Dum07t10&            &         &            &         &   -0.052*  &  (0.027)&   -0.051*  &  (0.030)\\ 
\addlinespace
Housing supply elasticity x Dum00t06&            &         &            &         &   -0.000   &  (0.002)&    0.000   &  (0.002)\\ 
\addlinespace
Housing supply elasticity x Dum07t10&            &         &            &         &    0.001   &  (0.004)&   -0.000   &  (0.004)\\ 
\addlinespace
House Vacancy Rate (1999) x Dum00t06&            &         &            &         &    0.239   &  (0.153)&    0.230   &  (0.150)\\ 
\addlinespace
House Vacancy Rate (1999) x Dum07t10&            &         &            &         &   -0.032   &  (0.083)&   -0.028   &  (0.085)\\ 
\addlinespace
Ratio of Renters (1999) x Dum00t06&            &         &            &         &   -0.123   &  (0.092)&   -0.141   &  (0.103)\\ 
\addlinespace
Ratio of Renters (1999) x Dum07t10&            &         &            &         &   -0.017   &  (0.038)&   -0.016   &  (0.049)\\ 
\addlinespace
Ratio of Bachelor Educated (1999) x Dum00t06&            &         &            &         &            &         &   -0.005   &  (0.064)\\ 
\addlinespace
Ratio of Bachelor Educated (1999) x Dum07t10&            &         &            &         &            &         &   -0.002   &  (0.076)\\ 
\addlinespace
Ratio of White Race (1999) x Dum00t06&            &         &            &         &            &         &   -0.005   &  (0.016)\\ 
\addlinespace
Ratio of White Race (1999) x Dum07t10&            &         &            &         &            &         &   -0.026   &  (0.025)\\ 
\addlinespace
Ratio of Immigration (90-00) x Dum00t06&            &         &            &         &            &         &    0.110   &  (0.090)\\ 
\addlinespace
Ratio of Immigration (90-00) x Dum07t10&            &         &            &         &            &         &   -0.147   &  (0.115)\\ 
\addlinespace
\midrule
Obs            &     1548   &         &     1548   &         &     1367   &         &     1367   &         \\
Cluster SE     &     CBSA   &         &     CBSA   &         &     CBSA   &         &     CBSA   &         \\
Weight         & Ln(HU99)   &         & Ln(HU99)   &         & Ln(HU99)   &         & Ln(HU99)   &         \\
KP F-Stat (99-05, non-stack sample)       &    23.12   &         &    21.09   &         &    13.79   &         &    11.63   &         \\
MOP F-Stat (99-05, non-stack sample)  &    22.05   &         &    20.35   &         &    13.82   &         &    11.66   &         \\
CoefEqual\_Chi2 &    0.134   &         &    0.363   &         &    0.606   &         &    0.473   &         \\
CoefEqual\_PValue &    0.714   &         &    0.547   &         &    0.436   &         &    0.492   &         \\
\bottomrule

\end{tabular}

} % end of resize box

\end{table}

==> Table_Purch/table_GSEM.D99t05vsD05t08.2SLS.tex <==
%----------------------------------------------------------------

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% table_GSEM.D99t05vsD05t08.2SLS
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\noindent 

\begin{table}[h!]
\centering
\caption{
\textbf{2SLS Stacked Regression of GSEM Growth in Boom (99-05) and Bust (05-08) Periods on Net Export Growth (99-05)} \smallskip \newline
{\scriptsize 
This table reports 2SLS stacked regression $\triangle_{99,05} \&  \triangle_{05,08}  Ln(GSEM_{c}) = \beta_{99,05} * \triangle_{99,05} \text{NetExp}_{m} \times Dum_{99,05} + \beta_{05,08} * \triangle_{99,05} \text{NetExp}_{m} \times Dum_{05,08} + \gamma_{99,05}* \bm{Controls_{c}} \times Dum_{99,05} + \gamma_{05,08}* \bm{Controls_{c}} \times Dum_{05,08}  + \alpha_{99,05} + \alpha_{05,08} + \epsilon_{period, c}$. The left-hand-side dependent variable $\triangle_{99,05} \& \triangle_{05,08} Ln(GSEM_{c})$ is the stacked growth rate of the dollar amount of government-sponsored enterprise mortgages (GSEMs) at county $c$ 99-05 and 05-08. The key independent variable $\triangle_{99,05} \text{NetExp}_{m} $ is the growth rate of net export at the metropolitan area (CBSA03 code) $m$ 99-05. $Controls_{c}$ indicates control variables at county $c$ in the period start year 1999. We use the gravity model-based instrumental variable $\triangle_{99,05}\text{givNetExp}_{m} \times Dum_{99,05} $ and $\triangle_{99,05}\text{givNetExp}_{m} \times Dum_{05,08} $ as IVs for $\triangle_{99,05}\text{NetExp}_{m} \times Dum_{99,05}$ and $\triangle_{99,05}\text{NetExp}_{m} \times Dum_{05,08}$. Each regression is weighted by the natural logarithm of housing units in the start year 1999. For the first-stage F-test of two non-stack samples, we report Kleibergen-Paap (2006) robust (clustered) statistics and Montiel Olea-Pflueger (2013) efficient statistics. We report Standard errors are clustered at the CBSA level. ***, **, and * indicate significance at the 1\%, 5\%, and 10\% levels, respectively.
} % end of small font size
} % end of caption
\label{table_GSEM.D99t05vsD05t08.2SLS}


\resizebox{0.95\columnwidth}{!}{%


\begin{tabular}{l*{6}{c}}
\toprule
\textbf{TSLS estimates}            &\multicolumn{5}{c}{GSEM Growth (99-05 and 05-08, annualized)} \\
            \cmidrule{2-6} 
            &\multicolumn{1}{c}{(1)}&\multicolumn{1}{c}{(2)}&\multicolumn{1}{c}{(3)}&\multicolumn{1}{c}{(4)}&\multicolumn{1}{c}{(5)}\\
            
\midrule
Net Export Growth (99-05, An) x Dum99t05&   14.987***&   14.110***&   13.820***&   13.817***&   13.356***\\
               &  (3.582)   &  (3.505)   &  (3.437)   &  (3.412)   &  (3.508)   \\
\addlinespace
Net Export Growth (99-05, An) x Dum05t08&  -14.713** &  -13.133** &  -13.704** &  -13.223** &  -10.991** \\
               &  (5.935)   &  (5.994)   &  (6.165)   &  (6.047)   &  (5.062)   \\
\addlinespace
Dummry 99-05   &    0.165***&    0.023   &   -0.203   &   -0.139   &   -0.061   \\
               &  (0.008)   &  (0.047)   &  (0.236)   &  (0.236)   &  (0.255)   \\
\addlinespace
Dummry 05-08   &   -0.394***&   -0.175** &   -0.464   &   -0.573*  &   -1.283***\\
               &  (0.017)   &  (0.075)   &  (0.319)   &  (0.308)   &  (0.326)   \\
\addlinespace
Ln(Num HH, 99) x Dum99t05&            &    0.013***&    0.011***&    0.038   &    0.047*  \\
               &            &  (0.004)   &  (0.003)   &  (0.026)   &  (0.028)   \\
\addlinespace
Ln(Num HH, 05) x Dum05t08&            &   -0.019***&   -0.021***&   -0.082   &   -0.044   \\
               &            &  (0.006)   &  (0.006)   &  (0.067)   &  (0.061)   \\
\addlinespace
Ln(HH Income, 99) x Dum99t05&            &            &    0.023   &    0.017   &    0.012   \\
               &            &            &  (0.020)   &  (0.020)   &  (0.022)   \\
\addlinespace
Ln(HH Income, 05) x Dum05t08&            &            &    0.028   &    0.037   &    0.088***\\
               &            &            &  (0.030)   &  (0.027)   &  (0.029)   \\
\addlinespace
Ln(Num of HH, 99) x Dum99t05&            &            &            &   -0.027   &   -0.037   \\
               &            &            &            &  (0.027)   &  (0.028)   \\
\addlinespace
Ln(Num of HH, 05) x Dum05t08&            &            &            &    0.061   &    0.031   \\
               &            &            &            &  (0.070)   &  (0.064)   \\
\addlinespace
Housing supply elasticity x Dum99t05&            &            &            &            &   -0.007*  \\
               &            &            &            &            &  (0.004)   \\
\addlinespace
Housing supply elasticity x Dum05t08&            &            &            &            &    0.035***\\
               &            &            &            &            &  (0.007)   \\
\midrule
Obs            &     1584   &     1584   &     1584   &     1584   &     1402   \\
Cluster SE     &     CBSA   &     CBSA   &     CBSA   &     CBSA   &     CBSA   \\
Weight         & {\scriptsize Ln(HU-Start)}   & {\scriptsize Ln(HU-Start)}   &{\scriptsize Ln(HU-Start)}   &{\scriptsize Ln(HU-Start)}   &{\scriptsize Ln(HU-Start)}    \\
Kleibergen-Paap F-Stat (99-05, Non-stack Sample)  &    23.36   &    23.24   &    23.02   &    23.33   &    16.88   \\
MOP F-Eff (99-05, Non-stack Sample) &    22.91   &    22.74   &    22.55   &    22.85   &    16.52   \\
CoefEqual\_Chi2 &   11.758   &    9.916   &    9.720   &    9.722   &   10.102   \\
CoefEqual\_PValue&    0.001   &    0.002   &    0.002   &    0.002   &    0.001   \\
\bottomrule

\end{tabular}

} % end of resize box

\end{table}


==> Table_Purch/table_GSEM.D99t05vsD05t08.2SLS.wide.tex <==
%----------------------------------------------------------------

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% table_GSEM.D99t05vsD05t08.2SLS.wide
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\noindent 

\begin{table}[h!]
\centering
\caption{
\textbf{2SLS Stacked Regression of GSEM Growth in Boom (99-05) and Bust (05-08) Periods on Net Export Growth (99-05)} \smallskip \newline
{\scriptsize 
This table reports 2SLS stacked regression $\triangle_{99,05} \&  \triangle_{05,08}  Ln(GSEM_{c}) = \beta_{99,05} * \triangle_{99,05} \text{NetExp}_{m} \times Dum_{99,05} + \beta_{05,08} * \triangle_{99,05} \text{NetExp}_{m} \times Dum_{05,08} + \gamma_{99,05}* \bm{Controls_{c}} \times Dum_{99,05} + \gamma_{05,08}* \bm{Controls_{c}} \times Dum_{05,08}  + \alpha_{99,05} + \alpha_{05,08} + \epsilon_{period, c}$. The left-hand-side dependent variable $\triangle_{99,05} \& \triangle_{05,08} Ln(GSEM_{c})$ is the stacked growth rate of the dollar amount of government-sponsored enterprise mortgages (GSEMs) at county $c$ 99-05 and 05-08. The key independent variable $\triangle_{99,05} \text{NetExp}_{m} $ is the growth rate of net export at the metropolitan area (CBSA03 code) $m$ 99-05. $Controls_{c}$ indicates control variables at county $c$ in the period start year 1999. We use the gravity model-based instrumental variable $\triangle_{99,05}\text{givNetExp}_{m} \times Dum_{99,05} $ and $\triangle_{99,05}\text{givNetExp}_{m} \times Dum_{05,08} $ as IVs for $\triangle_{99,05}\text{NetExp}_{m} \times Dum_{99,05}$ and $\triangle_{99,05}\text{NetExp}_{m} \times Dum_{05,08}$. Each regression is weighted by the natural logarithm of housing units in the start year 1999. For the first-stage F-test of two non-stack samples, we report Kleibergen-Paap (2006) robust (clustered) statistics and Montiel Olea-Pflueger (2013) efficient statistics. We report Standard errors are clustered at the CBSA level. ***, **, and * indicate significance at the 1\%, 5\%, and 10\% levels, respectively.
} % end of small font size
} % end of caption
\label{table_GSEM.D99t05vsD05t08.2SLS.wide}


\resizebox{0.95\columnwidth}{!}{%


\begin{tabular}{l*{8}{c}}
\toprule
\textbf{TSLS estimates}            &\multicolumn{8}{c}{GSEM Growth (99-05 and 05-08, annualized)} \\
            \cmidrule{2-9} 
            &\multicolumn{2}{c}{(1)}&\multicolumn{2}{c}{(2)}&\multicolumn{2}{c}{(3)}&\multicolumn{2}{c}{(4)}\\
            
\midrule
Net Export Growth (99-05, An) x Dum99t05&    1.889   &  (2.539)&    4.626** &  (2.265)&    3.071   &  (2.329)&    3.149   &  (2.307)\\ 
\addlinespace
Net Export Growth (99-05, An) x Dum05t08&   -3.514   &  (4.956)&   -6.394   &  (4.648)&   -7.124   &  (5.245)&   -4.614   &  (5.172)\\ 
\addlinespace
Dummry 99-05   &    0.046***&  (0.008)&    1.074***&  (0.187)&    0.851***&  (0.207)&    1.216***&  (0.329)\\ 
\addlinespace
Dummry 05-08   &   -0.080***&  (0.017)&   -1.479** &  (0.622)&   -1.677***&  (0.606)&   -0.456   &  (0.688)\\ 
\addlinespace
Ln(Num of HH, 99) x pd\_D99t05&            &         &   -0.015***&  (0.002)&    0.011   &  (0.036)&    0.054   &  (0.034)\\ 
\addlinespace
Ln(Num of HH, 99) x pd\_D05t08&            &         &    0.014** &  (0.006)&    0.020   &  (0.088)&   -0.068   &  (0.084)\\ 
\addlinespace
Ln(HH Income, 99) x pd\_D99t05&            &         &   -0.067***&  (0.020)&   -0.049** &  (0.023)&   -0.090***&  (0.033)\\ 
\addlinespace
Ln(HH Income, 99) x pd\_D05t08&            &         &    0.121*  &  (0.066)&    0.167** &  (0.069)&    0.071   &  (0.074)\\ 
\addlinespace
Ratio of Labor Force (1999) x pd\_D99t05&            &         &   -0.214***&  (0.075)&   -0.228** &  (0.091)&   -0.327***&  (0.084)\\ 
\addlinespace
Ratio of Labor Force (1999) x pd\_D05t08&            &         &   -0.090   &  (0.199)&   -0.281   &  (0.218)&   -0.094   &  (0.198)\\ 
\addlinespace
Ln(Num of HU, 99) x pd\_D99t05&            &         &            &         &   -0.023   &  (0.037)&   -0.065*  &  (0.035)\\ 
\addlinespace
Ln(Num of HU, 99) x pd\_D05t08&            &         &            &         &   -0.036   &  (0.088)&    0.040   &  (0.085)\\ 
\addlinespace
Housing supply elasticity x pd\_D99t05&            &         &            &         &    0.002   &  (0.003)&    0.002   &  (0.003)\\ 
\addlinespace
Housing supply elasticity x pd\_D05t08&            &         &            &         &   -0.005   &  (0.006)&   -0.002   &  (0.005)\\ 
\addlinespace
House Vacancy Rate (1999) x pd\_D99t05&            &         &            &         &    0.216** &  (0.093)&    0.247***&  (0.094)\\ 
\addlinespace 
House Vacancy Rate (1999) x pd\_D05t08&            &         &            &         &   -0.145   &  (0.138)&   -0.276*  &  (0.144)\\ 
\addlinespace
Ratio of Renters (1999) x pd\_D99t05&            &         &            &         &   -0.032   &  (0.061)&    0.045   &  (0.061)\\ 
\addlinespace
Ratio of Renters (1999) x pd\_D05t08&            &         &            &         &    0.586***&  (0.145)&    0.159   &  (0.104)\\ 
\addlinespace
Ratio of Bachelor Educated (1999) x pd\_D99t05&            &         &            &         &            &         &    0.172** &  (0.083)\\ 
\addlinespace
Ratio of Bachelor Educated (1999) x pd\_D05t08&            &         &            &         &            &         &    0.147   &  (0.153)\\ 
\addlinespace
Ratio of White Race (1999) x pd\_D99t05&            &         &            &         &            &         &    0.085***&  (0.024)\\ 
\addlinespace
Ratio of White Race (1999) x pd\_D05t08&            &         &            &         &            &         &   -0.145***&  (0.048)\\ 
\addlinespace
Ratio of Immigration (90-00) x pd\_D99t05&            &         &            &         &            &         &   -0.326   &  (0.202)\\ 
\addlinespace
Ratio of Immigration (90-00) x pd\_D05t08&            &         &            &         &            &         &    1.767***&  (0.477)\\ 
\addlinespace

\midrule
Obs            &     1584   &         &     1584   &         &     1402   &         &     1402   &         \\
Cluster SE     &     CBSA   &         &     CBSA   &         &     CBSA   &         &     CBSA   &         \\
Weight         & Ln(HU99)   &         & Ln(HU99)   &         & Ln(HU99)   &         & Ln(HU99)   &         \\
KP F-Stat      &    23.36   &         &    23.11   &         &    16.44   &         &    17.78   &         \\
MOP F-Eff      &    22.91   &         &    22.63   &         &    16.08   &         &    17.44   &         \\
CoefEqual\_Chi2 &    0.727   &         &    3.639   &         &    2.404   &         &    1.380   &         \\
CoefEqual\_PValue &    0.394   &         &    0.056   &         &    0.121   &         &    0.240   &         \\
\bottomrule

\end{tabular}

} % end of resize box

\end{table}


==> Table_Purch/table_House.D00t06vsD07t10.PLMNJ.2SLS..tex <==
%-----------------------------------------------------------------------
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% table_House.D00t06vsD07t10.PLMNJ.2SLS.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\noindent 

\begin{table}[h!]
\centering
\caption{
\textbf{2SLS Stacked Regression of House Employment Growth in Boom (00-06) and Bust (07-10) Periods on PLMNJ Growth (99-05)} \smallskip \newline
{\scriptsize
This table reports 2SLS regression $\triangle_{00,06} \& \triangle_{07,10} HouseEmpShr_{c} = \beta_{00,06} * \triangle_{99,05} Ln(PLMNJ_{c}) \times Dum_{00,06} + \beta_{07,10} * \triangle_{99,05} Ln(PLMNJ_{c}) \times Dum_{07,10} + \gamma_{00,06}* \bm{Controls_{c}} \times Dum_{00,06} + \gamma_{07,10}* \bm{Controls_{c}} \times Dum_{07,10} + \epsilon_{period, c}$. The left-hand-side dependent variable $\triangle_{00,06} \& \triangle_{07,10} HouseEmpShr_{c}$ is the change of the house employment share in working-age population at county $c$ 00-06 and 07-10. The key independent variable $\triangle_{99,05} Ln(PLMNJ_{c})$ is the growth rate of the dollar amount (07USD) of private-label mortgages (non-jumbo) at county $c$ 99-05. $Controls_{c}$ indicates control variables at county $c$ in the period start year 1999. We use the gravity model-based instrumental variable $\triangle_{99,05}\text{givNetExp}_{m}$ as the IV for $\triangle_{99,05}Ln(PLMNJ_{c})$. Regression is weighted by the natural logarithm of housing units in 1999.  For the first-stage F-test of two non-stacked samples, we report Kleibergen-Paap (2006) robust (clustered) statistics and Montiel Olea-Pflueger (2013) efficient statistics. Standard errors are clustered at the CBSA level. ***, **, and * indicate significance at the 1\%, 5\%, and 10\% levels, respectively.
\smallskip
} % end of small font size
} % end of caption
\label{table_House.D00t06vsD07t10.PLMNJ.2SLS.}

\vspace{-2mm}

\resizebox{0.55\columnwidth}{!}{%
\begin{tabular}{l*{4}{c}}
\toprule
\textbf{TSLS estimates}            &\multicolumn{4}{c}{House Employment Growth (00-06 and 07-10, An)} \\
            \cmidrule{2-5} 
            &\multicolumn{1}{c}{(1)}&\multicolumn{1}{c}{(2)}&\multicolumn{1}{c}{(3)}&\multicolumn{1}{c}{(4)}\\
            
\midrule
PLMNJ Growth (07USD, 99-05, An) x Dum00t06&    0.002   &    0.001   &    0.001   &    0.001   \\
               &  (0.003)   &  (0.003)   &  (0.003)   &  (0.003)   \\
\addlinespace
PLMNJ Growth (07USD, 99-05, An) x Dum07t10&   -0.014***&   -0.011** &   -0.013*  &   -0.015*  \\
               &  (0.005)   &  (0.005)   &  (0.007)   &  (0.008)   \\
\addlinespace
Dum00t06       &    0.001   &   -0.007***&   -0.005   &   -0.010   \\
               &  (0.000)   &  (0.002)   &  (0.003)   &  (0.006)   \\
\addlinespace
Dum07t10       &    0.001   &    0.023***&    0.028***&    0.010   \\
               &  (0.001)   &  (0.004)   &  (0.006)   &  (0.010)   \\
\addlinespace
Ln(Num of HH, 99) x Dum00t06&            &    0.000   &    0.001   &    0.000   \\
               &            &  (0.000)   &  (0.001)   &  (0.001)   \\
\addlinespace
Ln(Num of HH, 99) x Dum07t10&            &   -0.000   &    0.001   &    0.001   \\
               &            &  (0.000)   &  (0.001)   &  (0.001)   \\
\addlinespace
Ln(HH Income, 99) x Dum00t06&            &    0.001** &    0.000   &    0.001   \\
               &            &  (0.000)   &  (0.000)   &  (0.001)   \\
\addlinespace
Ln(HH Income, 99) x Dum07t10&            &   -0.002***&   -0.002***&   -0.001   \\
               &            &  (0.000)   &  (0.001)   &  (0.001)   \\
\addlinespace
Ratio of Labor Force (1999) x Dum00t06&            &   -0.001   &    0.001   &    0.001   \\
               &            &  (0.001)   &  (0.001)   &  (0.001)   \\
\addlinespace
Ratio of Labor Force (1999) x Dum07t10&            &    0.002   &    0.000   &    0.000   \\
               &            &  (0.002)   &  (0.002)   &  (0.002)   \\
\addlinespace
Ln(Num of HU, 99) x Dum00t06&            &            &   -0.000   &   -0.000   \\
               &            &            &  (0.001)   &  (0.001)   \\
\addlinespace
Ln(Num of HU, 99) x Dum07t10&            &            &   -0.001   &   -0.001   \\
               &            &            &  (0.001)   &  (0.001)   \\
\addlinespace
Housing supply elasticity x Dum00t06&            &            &   -0.000   &   -0.000   \\
               &            &            &  (0.000)   &  (0.000)   \\
\addlinespace
Housing supply elasticity x Dum07t10&            &            &   -0.000   &   -0.000   \\
               &            &            &  (0.000)   &  (0.000)   \\
\addlinespace
House Vacancy Rate (1999) x Dum00t06&            &            &    0.004** &    0.004** \\
               &            &            &  (0.002)   &  (0.002)   \\
\addlinespace
House Vacancy Rate (1999) x Dum07t10&            &            &   -0.002   &   -0.001   \\
               &            &            &  (0.003)   &  (0.003)   \\
\addlinespace
Ratio of Renters (1999) x Dum00t06&            &            &   -0.002   &   -0.002   \\
               &            &            &  (0.001)   &  (0.001)   \\
\addlinespace
Ratio of Renters (1999) x Dum07t10&            &            &   -0.001   &    0.003*  \\
               &            &            &  (0.001)   &  (0.001)   \\
\addlinespace
Ratio of Bachelor Educated (1999) x Dum00t06&            &            &            &   -0.002   \\
               &            &            &            &  (0.001)   \\
\addlinespace
Ratio of Bachelor Educated (1999) x Dum07t10&            &            &            &   -0.005*  \\
               &            &            &            &  (0.003)   \\
\addlinespace
Ratio of White Race (1999) x Dum00t06&            &            &            &   -0.000   \\
               &            &            &            &  (0.000)   \\
\addlinespace
Ratio of White Race (1999) x Dum07t10&            &            &            &    0.001   \\
               &            &            &            &  (0.001)   \\
\addlinespace
Ratio of Immigration (90-00) x Dum00t06&            &            &            &    0.002   \\
               &            &            &            &  (0.002)   \\
\addlinespace
Ratio of Immigration (90-00) x Dum07t10&            &            &            &   -0.010** \\
               &            &            &            &  (0.004)   \\
\midrule
Obs            &     1582   &     1582   &     1400   &     1400   \\
Cluster SE     &     CBSA   &     CBSA   &     CBSA   &     CBSA   \\
Weight         & Ln(HU99)   & Ln(HU99)   & Ln(HU99)   & Ln(HU99)   \\
KP F-Stat (99-05, non-stack sample)       &    23.45   &    21.09   &    14.26   &    11.92   \\
MOP F-Stat (99-05, non-stack sample)  &    22.30   &    20.30   &    14.35   &    11.99   \\
CoefEqual\_Chi2  &    5.980   &    3.317   &    2.648   &    2.924   \\
CoefEqual\_PValue  &    0.014   &    0.069   &    0.104   &    0.087   \\
\bottomrule

\end{tabular}

} % end of resize box

\end{table}

==> Table_Purch/table_Mortgage.D00t06vsD07t10.PLMNJ.2SLS.tex <==
%-----------------------------------------------------------------------
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% table_Mortgage.D00t06vsD07t10.PLMNJ.2SLS
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\noindent 

\begin{table}[h!]
\centering
\caption{
\textbf{2SLS Stacked Regression of Mortgage Employment Growth in Boom (00-06) and Bust (07-10) Periods on PLMNJ Growth (99-05)} \smallskip \newline
{\scriptsize
This table reports 2SLS regression $\triangle_{00,06} \& \triangle_{07,10} MortgageEmpShr_{c} = \beta_{00,06} * \triangle_{99,05} Ln(PLMNJ_{c}) \times Dum_{00,06} + \beta_{07,10} * \triangle_{99,05} Ln(PLMNJ_{c}) \times Dum_{07,10} + \gamma_{00,06}* \bm{Controls_{c}} \times Dum_{00,06} + \gamma_{07,10}* \bm{Controls_{c}} \times Dum_{07,10} + \epsilon_{period, c}$. The left-hand-side dependent variable $\triangle_{00,06} \& \triangle_{07,10} MortgageEmpShr_{c}$ is the change of the mortgage employment share in working-age population at county $c$ 00-06 and 07-10. To reduce the impact of outliers, the dependent variable is winsorized at 2\% and 98\% levels in each period. To make the coefficient more visible in the table, the mortgage employment share growth is multiplied by 100. The key independent variable $\triangle_{99,05} Ln(PLMNJ_{c})$ is the growth rate of the dollar amount (07USD) of private-label mortgages (non-jumbo) at county $c$ 99-05. $Controls_{c}$ indicates control variables at county $c$ in the period start year 1999. We use the gravity model-based instrumental variable $\triangle_{99,05}\text{givNetExp}_{m}$ as the IV for $\triangle_{99,05}Ln(PLMNJ_{c})$. Regression is weighted by the natural logarithm of housing units in 1999.  For the first-stage F-test of two non-stacked samples, we report Kleibergen-Paap (2006) robust (clustered) statistics and Montiel Olea-Pflueger (2013) efficient statistics. Standard errors are clustered at the CBSA level. ***, **, and * indicate significance at the 1\%, 5\%, and 10\% levels, respectively.
\smallskip
} % end of small font size
} % end of caption
\label{table_Mortgage.D00t06vsD07t10.PLMNJ.2SLS}

\vspace{-2mm}

\resizebox{0.55\columnwidth}{!}{%
\begin{tabular}{l*{4}{c}}
\toprule
\textbf{TSLS estimates}            &\multicolumn{4}{c}{Mortgage Employment Growth (00-06 and 07-10, An)} \\
            \cmidrule{2-5} 
            &\multicolumn{1}{c}{(1)}&\multicolumn{1}{c}{(2)}&\multicolumn{1}{c}{(3)}&\multicolumn{1}{c}{(4)}\\
            
\midrule
PLMNJ Growth (07USD, 99-05, An) x Dum00t06&    0.074** &    0.029   &    0.025   &    0.039   \\
               &  (0.030)   &  (0.028)   &  (0.039)   &  (0.039)   \\
\addlinespace
PLMNJ Growth (07USD, 99-05, An) x Dum07t10&   -0.113** &   -0.037   &   -0.094   &   -0.125   \\
               &  (0.053)   &  (0.055)   &  (0.096)   &  (0.119)   \\
\addlinespace
Dum00t06       &   -0.006   &   -0.199***&   -0.227***&   -0.172** \\
               &  (0.005)   &  (0.035)   &  (0.046)   &  (0.085)   \\
\addlinespace
Dum07t10       &    0.001   &    0.396***&    0.481***&    0.162   \\
               &  (0.009)   &  (0.048)   &  (0.076)   &  (0.131)   \\
\addlinespace
Ln(Num of HH, 99) x Dum00t06&            &    0.003***&   -0.005   &   -0.009   \\
               &            &  (0.001)   &  (0.008)   &  (0.009)   \\
\addlinespace
Ln(Num of HH, 99) x Dum07t10&            &   -0.006***&    0.011   &    0.009   \\
               &            &  (0.001)   &  (0.011)   &  (0.013)   \\
\addlinespace
Ln(HH Income, 99) x Dum00t06&            &    0.016***&    0.018***&    0.013*  \\
               &            &  (0.004)   &  (0.004)   &  (0.008)   \\
\addlinespace
Ln(HH Income, 99) x Dum07t10&            &   -0.032***&   -0.038***&   -0.010   \\
               &            &  (0.005)   &  (0.007)   &  (0.013)   \\
\addlinespace
Ratio of Labor Force (1999) x Dum00t06&            &   -0.011   &   -0.003   &    0.002   \\
               &            &  (0.016)   &  (0.020)   &  (0.022)   \\
\addlinespace
Ratio of Labor Force (1999) x Dum07t10&            &    0.009   &   -0.009   &    0.005   \\
               &            &  (0.022)   &  (0.025)   &  (0.031)   \\
\addlinespace
Ln(Num of HU, 99) x Dum00t06&            &            &    0.008   &    0.011   \\
               &            &            &  (0.008)   &  (0.010)   \\
\addlinespace
Ln(Num of HU, 99) x Dum07t10&            &            &   -0.016   &   -0.012   \\
               &            &            &  (0.011)   &  (0.014)   \\
\addlinespace
Housing supply elasticity x Dum00t06&            &            &    0.001   &    0.001   \\
               &            &            &  (0.001)   &  (0.001)   \\
\addlinespace
Housing supply elasticity x Dum07t10&            &            &   -0.001   &   -0.002   \\
               &            &            &  (0.002)   &  (0.002)   \\
\addlinespace
House Vacancy Rate (1999) x Dum00t06&            &            &    0.004   &   -0.004   \\
               &            &            &  (0.017)   &  (0.017)   \\
\addlinespace
House Vacancy Rate (1999) x Dum07t10&            &            &    0.022   &    0.041   \\
               &            &            &  (0.034)   &  (0.040)   \\
\addlinespace
Ratio of Renters (1999) x Dum00t06&            &            &    0.010   &   -0.003   \\
               &            &            &  (0.011)   &  (0.014)   \\
\addlinespace
Ratio of Renters (1999) x Dum07t10&            &            &   -0.036** &    0.001   \\
               &            &            &  (0.016)   &  (0.021)   \\
\addlinespace
Ratio of Bachelor Educated (1999) x Dum00t06&            &            &            &    0.009   \\
               &            &            &            &  (0.024)   \\
\addlinespace
Ratio of Bachelor Educated (1999) x Dum07t10&            &            &            &   -0.098** \\
               &            &            &            &  (0.043)   \\
\addlinespace
Ratio of White Race (1999) x Dum00t06&            &            &            &   -0.002   \\
               &            &            &            &  (0.008)   \\
\addlinespace
Ratio of White Race (1999) x Dum07t10&            &            &            &    0.007   \\
               &            &            &            &  (0.011)   \\
\addlinespace
Ratio of Immigration (90-00) x Dum00t06&            &            &            &    0.072   \\
               &            &            &            &  (0.046)   \\
\addlinespace
Ratio of Immigration (90-00) x Dum07t10&            &            &            &   -0.061   \\
               &            &            &            &  (0.054)   \\
\midrule
Obs            &     1311   &     1311   &     1150   &     1150   \\
Cluster SE     &     CBSA   &     CBSA   &     CBSA   &     CBSA   \\
Weight         & Ln(HU99)   & Ln(HU99)   & Ln(HU99)   & Ln(HU99)   \\
KP F-Stat (99-05, non-stack sample)       &    24.16   &    21.54   &    12.38   &    11.13   \\
MOP F-Stat (99-05, non-stack sample)  &    23.11   &    20.76   &    12.26   &    10.99   \\
CoefEqual\_Chi2 & 6.905   &    0.875   &    0.940   &    1.241   \\
CoefEqual\_PValue &    0.009   &    0.350   &    0.332   &    0.265   \\
\bottomrule

\end{tabular}

} % end of resize box

\end{table}

==> Table_Purch/table_Mortgage.D00t06vsD07t10.PLMNJ.2SLS.wide.tex <==
%-----------------------------------------------------------------------
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% table_Mortgage.D00t06vsD07t10.PLMNJ.2SLS.wide
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\noindent 

\begin{table}[h!]
\centering
\caption{
\textbf{2SLS Stacked Regression of Mortgage Employment Growth in Boom (00-06) and Bust (07-10) Periods on PLMNJ Growth (99-05)} \smallskip \newline
{\scriptsize
This table reports 2SLS regression $\triangle_{00,06} \& \triangle_{07,10} MortgageEmpShr_{c} = \beta_{00,06} * \triangle_{99,05} Ln(PLMNJ_{c}) \times Dum_{00,06} + \beta_{07,10} * \triangle_{99,05} Ln(PLMNJ_{c}) \times Dum_{07,10} + \gamma_{00,06}* \bm{Controls_{c}} \times Dum_{00,06} + \gamma_{07,10}* \bm{Controls_{c}} \times Dum_{07,10} + \epsilon_{period, c}$. The left-hand-side dependent variable $\triangle_{00,06} \& \triangle_{07,10} MortgageEmpShr_{c}$ is the change of the mortgage employment share in working-age population at county $c$ 00-06 and 07-10. To reduce the impact of outliers, the dependent variable is winsorized at 2\% and 98\% levels in each period. To make the coefficient more visible in the table, the mortgage employment share growth is multiplied by 100. The key independent variable $\triangle_{99,05} Ln(PLMNJ_{c})$ is the growth rate of the dollar amount (07USD) of private-label mortgages (non-jumbo) at county $c$ 99-05. $Controls_{c}$ indicates control variables at county $c$ in the period start year 1999. We use the gravity model-based instrumental variable $\triangle_{99,05}\text{givNetExp}_{m}$ as the IV for $\triangle_{99,05}Ln(PLMNJ_{c})$. Regression is weighted by the natural logarithm of housing units in 1999.  For the first-stage F-test of two non-stacked samples, we report Kleibergen-Paap (2006) robust (clustered) statistics and Montiel Olea-Pflueger (2013) efficient statistics. Standard errors are clustered at the CBSA level. ***, **, and * indicate significance at the 1\%, 5\%, and 10\% levels, respectively.
\smallskip
} % end of small font size
} % end of caption
\label{table_Mortgage.D00t06vsD07t10.PLMNJ.2SLS.wide}

\vspace{-2mm}

\resizebox{\columnwidth}{!}{%
\begin{tabular}{l*{8}{c}}
\toprule
\textbf{TSLS estimates}            &\multicolumn{8}{c}{Other House Employment Growth (00-06 and 07-10, An)} \\
            \cmidrule{2-9} 
            &\multicolumn{2}{c}{(1)}&\multicolumn{2}{c}{(2)}&\multicolumn{2}{c}{(3)}&\multicolumn{2}{c}{(4)}\\
            
\midrule
PLMNJ Growth (07USD, 99-05, An) x Dum00t06&    0.074** &  (0.030)&    0.029   &  (0.028)&    0.025   &  (0.039)&    0.039   &  (0.039)\\ 
\addlinespace
PLMNJ Growth (07USD, 99-05, An) x Dum07t10&   -0.113** &  (0.053)&   -0.037   &  (0.055)&   -0.094   &  (0.096)&   -0.125   &  (0.119)\\ 
\addlinespace
Dum00t06       &   -0.006   &  (0.005)&   -0.199***&  (0.035)&   -0.227***&  (0.046)&   -0.172** &  (0.085)\\ 
\addlinespace
Dum07t10       &    0.001   &  (0.009)&    0.396***&  (0.048)&    0.481***&  (0.076)&    0.162   &  (0.131)\\ 
\addlinespace
Ln(Num of HH, 99) x Dum00t06&            &         &    0.003***&  (0.001)&   -0.005   &  (0.008)&   -0.009   &  (0.009)\\ 
\addlinespace
Ln(Num of HH, 99) x Dum07t10&            &         &   -0.006***&  (0.001)&    0.011   &  (0.011)&    0.009   &  (0.013)\\ 
\addlinespace
Ln(HH Income, 99) x Dum00t06&            &         &    0.016***&  (0.004)&    0.018***&  (0.004)&    0.013*  &  (0.008)\\ 
\addlinespace
Ln(HH Income, 99) x Dum07t10&            &         &   -0.032***&  (0.005)&   -0.038***&  (0.007)&   -0.010   &  (0.013)\\ 
\addlinespace
Ratio of Labor Force (1999) x Dum00t06&            &         &   -0.011   &  (0.016)&   -0.003   &  (0.020)&    0.002   &  (0.022)\\ 
\addlinespace
Ratio of Labor Force (1999) x Dum07t10&            &         &    0.009   &  (0.022)&   -0.009   &  (0.025)&    0.005   &  (0.031)\\ 
\addlinespace
Ln(Num of HU, 99) x Dum00t06&            &         &            &         &    0.008   &  (0.008)&    0.011   &  (0.010)\\ 
\addlinespace
Ln(Num of HU, 99) x Dum07t10&            &         &            &         &   -0.016   &  (0.011)&   -0.012   &  (0.014)\\ 
\addlinespace
Housing supply elasticity x Dum00t06&            &         &            &         &    0.001   &  (0.001)&    0.001   &  (0.001)\\ 
\addlinespace
Housing supply elasticity x Dum07t10&            &         &            &         &   -0.001   &  (0.002)&   -0.002   &  (0.002)\\ 
\addlinespace
House Vacancy Rate (1999) x Dum00t06&            &         &            &         &    0.004   &  (0.017)&   -0.004   &  (0.017)\\ 
\addlinespace
House Vacancy Rate (1999) x Dum07t10&            &         &            &         &    0.022   &  (0.034)&    0.041   &  (0.040)\\ 
\addlinespace
Ratio of Renters (1999) x Dum00t06&            &         &            &         &    0.010   &  (0.011)&   -0.003   &  (0.014)\\ 
\addlinespace
Ratio of Renters (1999) x Dum07t10&            &         &            &         &   -0.036** &  (0.016)&    0.001   &  (0.021)\\ 
\addlinespace
Ratio of Bachelor Educated (1999) x Dum00t06&            &         &            &         &            &         &    0.009   &  (0.024)\\ 
\addlinespace
Ratio of Bachelor Educated (1999) x Dum07t10&            &         &            &         &            &         &   -0.098** &  (0.043)\\ 
\addlinespace
Ratio of White Race (1999) x Dum00t06&            &         &            &         &            &         &   -0.002   &  (0.008)\\ 
\addlinespace
Ratio of White Race (1999) x Dum07t10&            &         &            &         &            &         &    0.007   &  (0.011)\\ 
\addlinespace
Ratio of Immigration (90-00) x Dum00t06&            &         &            &         &            &         &    0.072   &  (0.046)\\ 
\addlinespace
Ratio of Immigration (90-00) x Dum07t10&            &         &            &         &            &         &   -0.061   &  (0.054)\\ 
\addlinespace
\midrule
Obs            &     1311   &         &     1311   &         &     1150   &         &     1150   &         \\
Cluster SE     &     CBSA   &         &     CBSA   &         &     CBSA   &         &     CBSA   &         \\
Weight         & Ln(HU99)   &         & Ln(HU99)   &         & Ln(HU99)   &         & Ln(HU99)   &         \\
KP F-Stat (99-05, non-stack sample)      &    24.16   &         &    21.54   &         &    12.38   &         &    11.13   &         \\
MOP F-Stat (99-05, non-stack sample)  &    23.11   &         &    20.76   &         &    12.26   &         &    10.99   &         \\
CoefEqual\_Chi2 &    6.905   &         &    0.875   &         &    0.940   &         &    1.241   &         \\
CoefEqual\_PValue &    0.009   &         &    0.350   &         &    0.332   &         &    0.265   &         \\
\bottomrule

\end{tabular}

} % end of resize box

\end{table}

==> Table_Purch/table_Other.D00t06vsD07t10.PLMNJ.2SLS.tex <==
%-----------------------------------------------------------------------
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% table_Other.D00t06vsD07t10.PLMNJ.2SLS
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\noindent 

\begin{table}[h!]
\centering
\caption{
\textbf{2SLS Stacked Regression of Other House Employment Growth in Boom (00-06) and Bust (07-10) Periods on PLMNJ Growth (99-05)} \smallskip \newline
{\scriptsize
This table reports 2SLS regression $\triangle_{00,06} \& \triangle_{07,10} OtherHouseEmpShr_{c} = \beta_{00,06} * \triangle_{99,05} Ln(PLMNJ_{c}) \times Dum_{00,06} + \beta_{07,10} * \triangle_{99,05} Ln(PLMNJ_{c}) \times Dum_{07,10} + \gamma_{00,06}* \bm{Controls_{c}} \times Dum_{00,06} + \gamma_{07,10}* \bm{Controls_{c}} \times Dum_{07,10} + \epsilon_{period, c}$. The left-hand-side dependent variable $\triangle_{00,06} \& \triangle_{07,10} OtherHouseEmpShr_{c}$ is the change of the other house employment share in working-age population at county $c$ 00-06 and 07-10. To reduce the impact of outliers, the dependent variable is winsorized at 5\% and 95\% levels in each period. To make the coefficient more visible in the table, the other employment share growth is multiplied by 100. The key independent variable $\triangle_{99,05} Ln(PLMNJ_{c})$ is the growth rate of the dollar amount (07USD) of private-label mortgages (non-jumbo) at county $c$ 99-05. $Controls_{c}$ indicates control variables at county $c$ in the period start year 1999. We use the gravity model-based instrumental variable $\triangle_{99,05}\text{givNetExp}_{m}$ as the IV for $\triangle_{99,05}Ln(PLMNJ_{c})$. Regression is weighted by the natural logarithm of housing units in 1999.  For the first-stage F-test of two non-stacked samples, we report Kleibergen-Paap (2006) robust (clustered) statistics and Montiel Olea-Pflueger (2013) efficient statistics. Standard errors are clustered at the CBSA level. ***, **, and * indicate significance at the 1\%, 5\%, and 10\% levels, respectively.
\smallskip
} % end of small font size
} % end of caption
\label{table_Other.D00t06vsD07t10.PLMNJ.2SLS}

\vspace{-2mm}

\resizebox{0.55\columnwidth}{!}{%
\begin{tabular}{l*{4}{c}}
\toprule
\textbf{TSLS estimates}            &\multicolumn{4}{c}{Other House Employment Growth (00-06 and 07-10, An)} \\
            \cmidrule{2-5} 
            &\multicolumn{1}{c}{(1)}&\multicolumn{1}{c}{(2)}&\multicolumn{1}{c}{(3)}&\multicolumn{1}{c}{(4)}\\
            
\midrule
PLMNJ Growth (07USD, 99-05, An) x Dum00t06&    0.204***&    0.175***&    0.164** &    0.189** \\
               &  (0.068)   &  (0.066)   &  (0.083)   &  (0.084)   \\
\addlinespace
PLMNJ Growth (07USD, 99-05, An) x Dum07t10&   -0.358***&   -0.284***&   -0.305** &   -0.350** \\
               &  (0.107)   &  (0.101)   &  (0.138)   &  (0.145)   \\
\addlinespace
Dum00t06       &   -0.006   &   -0.181***&   -0.105   &   -0.006   \\
               &  (0.011)   &  (0.070)   &  (0.082)   &  (0.134)   \\
\addlinespace
Dum07t10       &    0.013   &    0.390***&    0.334** &    0.119   \\
               &  (0.018)   &  (0.104)   &  (0.137)   &  (0.197)   \\
\addlinespace
Ln(Num of HH, 99) x Dum00t06&            &    0.001   &   -0.012   &   -0.022*  \\
               &            &  (0.001)   &  (0.012)   &  (0.013)   \\
\addlinespace
Ln(Num of HH, 99) x Dum07t10&            &   -0.006***&    0.016   &    0.035*  \\
               &            &  (0.002)   &  (0.017)   &  (0.019)   \\
\addlinespace
Ln(HH Income, 99) x Dum00t06&            &    0.014*  &    0.006   &   -0.002   \\
               &            &  (0.007)   &  (0.008)   &  (0.013)   \\
\addlinespace
Ln(HH Income, 99) x Dum07t10&            &   -0.028** &   -0.020   &   -0.003   \\
               &            &  (0.011)   &  (0.014)   &  (0.020)   \\
\addlinespace
Ratio of Labor Force (1999) x Dum00t06&            &    0.026   &    0.029   &    0.048   \\
               &            &  (0.027)   &  (0.028)   &  (0.030)   \\
\addlinespace
Ratio of Labor Force (1999) x Dum07t10&            &   -0.030   &   -0.065   &   -0.099** \\
               &            &  (0.042)   &  (0.044)   &  (0.047)   \\
\addlinespace
Ln(Num of HU, 99) x Dum00t06&            &            &    0.015   &    0.024*  \\
               &            &            &  (0.012)   &  (0.013)   \\
\addlinespace
Ln(Num of HU, 99) x Dum07t10&            &            &   -0.024   &   -0.040** \\
               &            &            &  (0.017)   &  (0.019)   \\
\addlinespace
Housing supply elasticity x Dum00t06&            &            &   -0.000   &    0.000   \\
               &            &            &  (0.001)   &  (0.002)   \\
\addlinespace
Housing supply elasticity x Dum07t10&            &            &    0.000   &   -0.001   \\
               &            &            &  (0.003)   &  (0.003)   \\
\addlinespace
House Vacancy Rate (1999) x Dum00t06&            &            &   -0.031   &   -0.049   \\
               &            &            &  (0.039)   &  (0.038)   \\
\addlinespace
House Vacancy Rate (1999) x Dum07t10&            &            &   -0.002   &    0.032   \\
               &            &            &  (0.064)   &  (0.063)   \\
\addlinespace
Ratio of Renters (1999) x Dum00t06&            &            &   -0.029*  &   -0.066***\\
               &            &            &  (0.017)   &  (0.021)   \\
\addlinespace
Ratio of Renters (1999) x Dum07t10&            &            &    0.050** &    0.126***\\
               &            &            &  (0.026)   &  (0.032)   \\
\addlinespace
Ratio of Bachelor Educated (1999) x Dum00t06&            &            &            &    0.008   \\
               &            &            &            &  (0.037)   \\
\addlinespace
Ratio of Bachelor Educated (1999) x Dum07t10&            &            &            &   -0.026   \\
               &            &            &            &  (0.049)   \\
\addlinespace
Ratio of White Race (1999) x Dum00t06&            &            &            &   -0.010   \\
               &            &            &            &  (0.013)   \\
\addlinespace
Ratio of White Race (1999) x Dum07t10&            &            &            &    0.026   \\
               &            &            &            &  (0.019)   \\
\addlinespace
Ratio of Immigration (90-00) x Dum00t06&            &            &            &    0.192** \\
               &            &            &            &  (0.079)   \\
\addlinespace
Ratio of Immigration (90-00) x Dum07t10&            &            &            &   -0.348***\\
               &            &            &            &  (0.119)   \\
\midrule
Obs            &     1572   &     1572   &     1390   &     1390   \\
Cluster SE     &     CBSA   &     CBSA   &     CBSA   &     CBSA   \\
Weight         & Ln(HU99)   & Ln(HU99)   & Ln(HU99)   & Ln(HU99)   \\
KP F-Stat (99-05, non-stack sample)       &    23.25   &    20.97   &    14.25   &    12.02   \\
MOP F-Stat (99-05, non-stack sample)  &    22.06   &    20.11   &    14.27   &    12.05   \\
CoefEqual\_Chi2  &   11.846   &    8.818   &    5.252   &    6.372   \\
CoefEqual\_PValue &    0.001   &    0.003   &    0.022   &    0.012   \\
\bottomrule

\end{tabular}

} % end of resize box

\end{table}

==> Table_Purch/table_PLMNJ.D99t05vsD05t08.2SLS.tex <==
%----------------------------------------------------------------

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% table_PLMNJ.D99t05vsD05t08.2SLS
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\noindent 

\begin{table}[h!]
\centering
\caption{
\textbf{2SLS Stacked Regression of PLMNJ Growth in Boom (99-05) and Bust (05-08) Periods on Net Export Growth (9-05)} \smallskip \newline
{\scriptsize 
This table reports 2SLS stacked regression $\triangle_{99,05} \& \triangle_{05,08} Ln(PLMNJ_{c}) = \beta_{99,05} * \triangle_{99,05} \text{NetExp}_{m} \times Dum_{99,05} + \beta_{05,08} * \triangle_{99,05} \text{NetExp}_{m} \times Dum_{05,08} + \gamma_{99,05}* \bm{Controls_{c}} \times Dum_{99,05} + \gamma_{05,08}* \bm{Controls_{c}} \times Dum_{05,08}  + \alpha_{99,05} + \alpha_{05,08} + \epsilon_{period, c}$. The left-hand-side dependent variable $\triangle_{99,05} \& \triangle_{05,08} Ln(PLMNJ_{c})$ is the stacked growth rate of the dollar amount (07USD) of private-label mortgages (non-jumbo) (PLMNJ) at county $c$ 99-05 and 05-08. The key independent variable $\triangle_{99,05} \text{NetExp}_{m}$ is the growth rate of net export at the metropolitan area (CBSA03 code) $m$ 99-05. $Controls_{c}$ indicates control variables at county $c$ in the period start year 1999. We use the gravity model-based instrumental variable $\triangle_{99,05}\text{givNetExp}_{m}$ as IVs for $\triangle_{99,05}\text{NetExp}_{m}$. Regression is weighted by the natural logarithm of housing units in the start year 1999. We report the statistics and p-values for the tests of coefficient equality between $\beta_{99,05}$ and $\beta_{05,08}$. For the first-stage F-test of two separate non-stack samples, we report kleibergen-Paap (2006) robust (clustered) statistics and Montiel Olea-Pflueger (2013) efficient statistics. Standard errors are clustered at the CBSA level. ***, **, and * indicate significance at the 1\%, 5\%, and 10\% levels, respectively.
} % end of small font size
} % end of caption
\label{table_PLMNJ.D99t05vsD05t08.2SLS}


\resizebox{0.95\columnwidth}{!}{%


\begin{tabular}{l*{4}{c}}
\toprule
\textbf{TSLS estimates}            &\multicolumn{4}{c}{PLMNJ Growth (99-05 and 05-08, annualized)} \\
            \cmidrule{2-5} 
            &\multicolumn{1}{c}{(1)}&\multicolumn{1}{c}{(2)}&\multicolumn{1}{c}{(3)}&\multicolumn{1}{c}{(4)}\\
            
\midrule
Net Export Growth (99-05, An) x Dum99t05&   13.694***&   13.365***&   11.145***&   10.851***\\
               &  (3.547)   &  (3.643)   &  (3.254)   &  (3.331)   \\
\addlinespace
Net Export Growth (99-05, An) x Dum05t08&  -16.325***&  -16.915***&  -13.335** &  -12.438** \\
               &  (6.194)   &  (6.457)   &  (5.782)   &  (5.669)   \\
\addlinespace
Dummry 99-05   &    0.200***&    0.181   &    0.352   &   -0.339   \\
               &  (0.009)   &  (0.212)   &  (0.236)   &  (0.371)   \\
\addlinespace
Dummry 05-08   &   -0.320***&   -1.010***&   -1.711***&   -0.022   \\
               &  (0.018)   &  (0.375)   &  (0.436)   &  (0.720)   \\
\addlinespace
Ln(Num of HH, 99) x pd\_D99t05&            &    0.006** &    0.021   &    0.003   \\
               &            &  (0.003)   &  (0.032)   &  (0.031)   \\
\addlinespace
Ln(Num of HH, 99) x pd\_D05t08&            &   -0.010   &    0.083   &    0.157*  \\
               &            &  (0.006)   &  (0.081)   &  (0.082)   \\
\addlinespace
Ln(HH Income, 99) x pd\_D99t05&            &   -0.004   &   -0.027   &    0.035   \\
               &            &  (0.022)   &  (0.025)   &  (0.036)   \\
\addlinespace
Ln(HH Income, 99) x pd\_D05t08&            &    0.077*  &    0.161***&   -0.001   \\
               &            &  (0.041)   &  (0.046)   &  (0.070)   \\
\addlinespace
Ratio of Labor Force (1999) x pd\_D99t05&            &   -0.021   &    0.081   &    0.127   \\
               &            &  (0.107)   &  (0.099)   &  (0.102)   \\
\addlinespace
Ratio of Labor Force (1999) x pd\_D05t08&            &   -0.043   &   -0.355   &   -0.534** \\
               &            &  (0.234)   &  (0.224)   &  (0.241)   \\
\addlinespace
Ln(Num of HU, 99) x pd\_D99t05&            &            &   -0.010   &    0.009   \\
               &            &            &  (0.033)   &  (0.032)   \\
\addlinespace
Ln(Num of HU, 99) x pd\_D05t08&            &            &   -0.105   &   -0.180** \\
               &            &            &  (0.081)   &  (0.082)   \\
\addlinespace
Housing supply elasticity x pd\_D99t05&            &            &   -0.011***&   -0.011***\\
               &            &            &  (0.003)   &  (0.003)   \\
\addlinespace
Housing supply elasticity x pd\_D05t08&            &            &    0.029***&    0.028***\\
               &            &            &  (0.007)   &  (0.007)   \\
\addlinespace
House Vacancy Rate (1999) x pd\_D99t05&            &            &    0.179** &    0.187** \\
               &            &            &  (0.087)   &  (0.084)   \\
\addlinespace
House Vacancy Rate (1999) x pd\_D05t08&            &            &   -0.143   &   -0.130   \\
               &            &            &  (0.184)   &  (0.181)   \\
\addlinespace
Ratio of Renters (1999) x pd\_D99t05&            &            &   -0.107** &   -0.054   \\
               &            &            &  (0.053)   &  (0.058)   \\
\addlinespace
Ratio of Renters (1999) x pd\_D05t08&            &            &    0.316** &    0.287*  \\
               &            &            &  (0.128)   &  (0.152)   \\
\addlinespace
Ratio of Bachelor Educated (1999) x pd\_D99t05&            &            &            &   -0.239** \\
               &            &            &            &  (0.094)   \\
\addlinespace
Ratio of Bachelor Educated (1999) x pd\_D05t08&            &            &            &    0.610***\\
               &            &            &            &  (0.176)   \\
\addlinespace
Ratio of White Race (1999) x pd\_D99t05&            &            &            &    0.018   \\
               &            &            &            &  (0.035)   \\
\addlinespace
Ratio of White Race (1999) x pd\_D05t08&            &            &            &    0.074   \\
               &            &            &            &  (0.075)   \\
\addlinespace
Ratio of Immigration (90-00) x pd\_D99t05&            &            &            &    0.138   \\
               &            &            &            &  (0.197)   \\
\addlinespace
Ratio of Immigration (90-00) x pd\_D05t08&            &            &            &   -0.407   \\
               &            &            &            &  (0.392)   \\
\midrule
Obs            &     1584   &     1584   &     1402   &     1402   \\
Cluster SE     &     CBSA   &     CBSA   &     CBSA   &     CBSA   \\
Weight         & Ln(HU99)   & Ln(HU99)   & Ln(HU99)   & Ln(HU99)   \\
KP F-Stat (99-05, Non-stack Sample)  &    23.36   &    23.11   &    16.44   &    17.78   \\
MOP F-Eff (99-05, Non-stack Sample) &    22.91   &    22.63   &    16.08   &    17.44   \\
CoefEqual\_Chi2 &   11.266   &   10.375   &    9.183   &    8.386   \\
CoefEqual\_PValue &    0.001   &    0.001   &    0.002   &    0.004   \\
\bottomrule

\end{tabular}

} % end of resize box

\end{table}


==> Table_Purch/table_PermitValue.D99t05vsD05t09.PLMNJ.2SLS.tex <==
%-----------------------------------------------------------------------
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% table_PermitValue.D99t05vsD05t09.PLMNJ.2SLS
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\noindent 

\begin{table}[h!]
\centering
\caption{
\textbf{2SLS Stacked Regression of Residential Units Permit Value Growth in Boom (99-05) and Bust (05-09) Periods on PLMNJ Growth (99-05)} \smallskip \newline
{\scriptsize
This table reports 2SLS regression $\triangle_{99,05} \& \triangle_{05,09} Ln(PermitValue_{c}) = \beta_{99,05} * \triangle_{99,05} Ln(PLMNJ_{c}) \times Dum_{99,05} + \beta_{05,09} * \triangle_{99,05} Ln(PLMNJ_{c}) \times Dum_{05,09} + \gamma_{99,05}* \bm{Controls_{c}} \times Dum_{99,05} + \gamma_{05,09}* \bm{Controls_{c}} \times Dum_{05,09} + \epsilon_{period, c}$. The left-hand-side dependent variable $\triangle_{99,05} \& \triangle_{05,09} Ln(PermitValue_{c})$ is the residential units permit value (by imputation by U.S. Census) growth at county $c$ 99-05 and 05-09. The key independent variable $\triangle_{99,05} Ln(PLMNJ_{c})$ is the growth rate of the dollar amount (07USD) of private-label mortgages (non-jumbo) at county $c$ 99-05. $Controls_{c}$ indicates control variables at county $c$ in the period start year 1999. We use the gravity model-based instrumental variable $\triangle_{99,05}\text{givNetExp}_{m}$ as the IV for $\triangle_{99,05}Ln(PLMNJ_{c})$. Regression is weighted by the natural logarithm of housing units in 1999.  For the first-stage F-test of two non-stacked samples, we report Kleibergen-Paap (2006) robust (clustered) statistics and Montiel Olea-Pflueger (2013) efficient statistics. Standard errors are clustered at the CBSA level. ***, **, and * indicate significance at the 1\%, 5\%, and 10\% levels, respectively.
\smallskip
} % end of small font size
} % end of caption
\label{table_PermitValue.D99t05vsD05t09.PLMNJ.2SLS}

\vspace{-2mm}

\resizebox{0.55\columnwidth}{!}{%
\begin{tabular}{l*{4}{c}}
\toprule
\textbf{TSLS estimates}            &\multicolumn{4}{c}{Residential Units Permit Value Growth (99-05 \& 05-09, An)} \\
            \cmidrule{2-5} 
            &\multicolumn{1}{c}{(1)}&\multicolumn{1}{c}{(2)}&\multicolumn{1}{c}{(3)}&\multicolumn{1}{c}{(4)}\\
            
\midrule
PLMNJ Growth (07USD, 99-05, An) x Dum99t05&    0.689***&    0.827***&    0.661***&    0.713***\\
               &  (0.184)   &  (0.200)   &  (0.252)   &  (0.264)   \\
\addlinespace
PLMNJ Growth (07USD, 99-05, An) x Dum05t09&   -1.588***&   -1.462***&   -1.660***&   -1.648***\\
               &  (0.480)   &  (0.485)   &  (0.638)   &  (0.577)   \\
\addlinespace
Dum99t05       &   -0.051   &    0.723***&    0.554***&    0.977***\\
               &  (0.032)   &  (0.196)   &  (0.187)   &  (0.375)   \\
\addlinespace
Dum05t09       &   -0.027   &    1.096***&    0.732*  &    2.240***\\
               &  (0.078)   &  (0.356)   &  (0.420)   &  (0.753)   \\
\addlinespace
Ln(Num of HH, 99) x Dum99t05&            &   -0.006   &    0.002   &   -0.026   \\
               &            &  (0.005)   &  (0.048)   &  (0.048)   \\
\addlinespace
Ln(Num of HH, 99) x Dum05t09&            &    0.000   &    0.031   &    0.117   \\
               &            &  (0.006)   &  (0.081)   &  (0.082)   \\
\addlinespace
Ln(HH Income, 99) x Dum99t05&            &   -0.056***&   -0.040** &   -0.071** \\
               &            &  (0.021)   &  (0.019)   &  (0.036)   \\
\addlinespace
Ln(HH Income, 99) x Dum05t09&            &   -0.116***&   -0.080** &   -0.223***\\
               &            &  (0.037)   &  (0.040)   &  (0.069)   \\
\addlinespace
Ratio of Labor Force (1999) x Dum99t05&            &   -0.208** &   -0.159*  &   -0.108   \\
               &            &  (0.085)   &  (0.094)   &  (0.089)   \\
\addlinespace
Ratio of Labor Force (1999) x Dum05t09&            &    0.151   &    0.116   &   -0.089   \\
               &            &  (0.193)   &  (0.200)   &  (0.225)   \\
\addlinespace
Ln(Num of HU, 99) x Dum99t05&            &            &   -0.013   &    0.010   \\
               &            &            &  (0.048)   &  (0.047)   \\
\addlinespace
Ln(Num of HU, 99) x Dum05t09&            &            &   -0.033   &   -0.116   \\
               &            &            &  (0.082)   &  (0.082)   \\
\addlinespace
Housing supply elasticity x Dum99t05&            &            &    0.000   &    0.001   \\
               &            &            &  (0.005)   &  (0.005)   \\
\addlinespace
Housing supply elasticity x Dum05t09&            &            &   -0.005   &   -0.006   \\
               &            &            &  (0.010)   &  (0.010)   \\
\addlinespace
House Vacancy Rate (1999) x Dum99t05&            &            &    0.159   &    0.105   \\
               &            &            &  (0.116)   &  (0.121)   \\
\addlinespace
House Vacancy Rate (1999) x Dum05t09&            &            &    0.288   &    0.315   \\
               &            &            &  (0.252)   &  (0.246)   \\
\addlinespace
Ratio of Renters (1999) x Dum99t05&            &            &    0.139*  &   -0.002   \\
               &            &            &  (0.084)   &  (0.090)   \\
\addlinespace
Ratio of Renters (1999) x Dum05t09&            &            &    0.123   &    0.144   \\
               &            &            &  (0.158)   &  (0.180)   \\
\addlinespace
Ratio of Bachelor Educated (1999) x Dum99t05&            &            &            &    0.081   \\
               &            &            &            &  (0.093)   \\
\addlinespace
Ratio of Bachelor Educated (1999) x Dum05t09&            &            &            &    0.612***\\
               &            &            &            &  (0.206)   \\
\addlinespace
Ratio of White Race (1999) x Dum99t05&            &            &            &   -0.080** \\
               &            &            &            &  (0.034)   \\
\addlinespace
Ratio of White Race (1999) x Dum05t09&            &            &            &    0.042   \\
               &            &            &            &  (0.128)   \\
\addlinespace
Ratio of Immigration (90-00) x Dum99t05&            &            &            &    0.393** \\
               &            &            &            &  (0.170)   \\
\addlinespace
Ratio of Immigration (90-00) x Dum05t09&            &            &            &   -0.898   \\
               &            &            &            &  (0.585)   \\
\midrule
Obs            &     1582   &     1582   &     1401   &     1401   \\
Cluster SE     &     CBSA   &     CBSA   &     CBSA   &     CBSA   \\
Weight         & Ln(HU99)   & Ln(HU99)   & Ln(HU99)   & Ln(HU99)   \\
KP F-Stat (99-05, non-stack sample)       &    23.43   &    21.04   &    13.97   &    11.74   \\
MOP F-Stat (99-05, non-stack sample)  &    22.30   &    20.29   &    14.03   &    11.80   \\
CoefEqual\_Chi2  &   16.078   &   14.832   &    9.361   &   10.906   \\
CoefEqual\_PValue &    0.000   &    0.000   &    0.002   &    0.001   \\
\bottomrule

\end{tabular}

} % end of resize box

\end{table}

==> Table_Purch/table_RefineHouse.D00t06vsD07t10.PLMNJ.2SLS.tex <==
%-----------------------------------------------------------------------
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% table_RefineHouse.D00t06vsD07t10.PLMNJ.2SLS
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\noindent 

\begin{table}[h!]
\centering
\caption{
\textbf{2SLS Stacked Regression of Refined House Employment Growth in Boom (00-06) and Bust (07-10) Periods on PLMNJ Growth (99-05)} \smallskip \newline
{\scriptsize
This table reports 2SLS regression $\triangle_{00,06} \& \triangle_{07,10} RefinedHouseEmpShr_{c} = \beta_{00,06} * \triangle_{99,05} Ln(PLMNJ_{c}) \times Dum_{00,06} + \beta_{07,10} * \triangle_{99,05} Ln(PLMNJ_{c}) \times Dum_{07,10} + \gamma_{00,06}* \bm{Controls_{c}} \times Dum_{00,06} + \gamma_{07,10}* \bm{Controls_{c}} \times Dum_{07,10} + \epsilon_{period, c}$. The left-hand-side dependent variable $\triangle_{00,06} \& \triangle_{07,10} RefinedHouseEmpShr_{c}$ is the change of the refined house employment share in working-age population at county $c$ 00-06 and 07-10. To reduce the impact of outliers, the dependent variable is winsorized at 2\% and 98\% levels in each period. To make the coefficient more visible in the table, the refined house employment share growth is multiplied by 100. The key independent variable $\triangle_{99,05} Ln(PLMNJ_{c})$ is the growth rate of the dollar amount (07USD) of private-label mortgages (non-jumbo) at county $c$ 99-05. $Controls_{c}$ indicates control variables at county $c$ in the period start year 1999. We use the gravity model-based instrumental variable $\triangle_{99,05}\text{givNetExp}_{m}$ as the IV for $\triangle_{99,05}Ln(PLMNJ_{c})$. Regression is weighted by the natural logarithm of housing units in 1999.  For the first-stage F-test of two non-stacked samples, we report Kleibergen-Paap (2006) robust (clustered) statistics and Montiel Olea-Pflueger (2013) efficient statistics. Standard errors are clustered at the CBSA level. ***, **, and * indicate significance at the 1\%, 5\%, and 10\% levels, respectively.
\smallskip
} % end of small font size
} % end of caption
\label{table_RefineHouse.D00t06vsD07t10.PLMNJ.2SLS}

\vspace{-2mm}

\resizebox{0.55\columnwidth}{!}{%
\begin{tabular}{l*{4}{c}}
\toprule
\textbf{TSLS estimates}            &\multicolumn{4}{c}{Refined House Employment Growth (00-06 and 07-10, An)} \\
            \cmidrule{2-5} 
            &\multicolumn{1}{c}{(1)}&\multicolumn{1}{c}{(2)}&\multicolumn{1}{c}{(3)}&\multicolumn{1}{c}{(4)}\\
            
\midrule
PLMNJ Growth (07USD, 99-05, An) x Dum00t06&    0.378***&    0.333***&    0.331** &    0.382** \\
               &  (0.123)   &  (0.125)   &  (0.163)   &  (0.170)   \\
\addlinespace
PLMNJ Growth (07USD, 99-05, An) x Dum07t10&   -0.693***&   -0.537***&   -0.591** &   -0.696** \\
               &  (0.195)   &  (0.193)   &  (0.264)   &  (0.309)   \\
\addlinespace
Dum00t06       &   -0.023   &   -0.432***&   -0.419***&   -0.265   \\
               &  (0.021)   &  (0.117)   &  (0.140)   &  (0.232)   \\
\addlinespace
Dum07t10       &    0.030   &    1.101***&    1.151***&    0.301   \\
               &  (0.034)   &  (0.182)   &  (0.250)   &  (0.372)   \\
\addlinespace
Ln(Num of HH, 99) x Dum00t06&            &    0.000   &   -0.019   &   -0.039*  \\
               &            &  (0.002)   &  (0.018)   &  (0.021)   \\
\addlinespace
Ln(Num of HH, 99) x Dum07t10&            &   -0.009***&    0.038   &    0.059*  \\
               &            &  (0.003)   &  (0.026)   &  (0.030)   \\
\addlinespace
Ln(HH Income, 99) x Dum00t06&            &    0.042***&    0.036** &    0.023   \\
               &            &  (0.012)   &  (0.014)   &  (0.023)   \\
\addlinespace
Ln(HH Income, 99) x Dum07t10&            &   -0.097***&   -0.088***&   -0.015   \\
               &            &  (0.020)   &  (0.025)   &  (0.037)   \\
\addlinespace
Ratio of Labor Force (1999) x Dum00t06&            &   -0.057   &   -0.007   &    0.030   \\
               &            &  (0.046)   &  (0.050)   &  (0.054)   \\
\addlinespace
Ratio of Labor Force (1999) x Dum07t10&            &    0.048   &   -0.070   &   -0.094   \\
               &            &  (0.077)   &  (0.080)   &  (0.091)   \\
\addlinespace
Ln(Num of HU, 99) x Dum00t06&            &            &    0.021   &    0.038*  \\
               &            &            &  (0.018)   &  (0.021)   \\
\addlinespace
Ln(Num of HU, 99) x Dum07t10&            &            &   -0.052** &   -0.066** \\
               &            &            &  (0.026)   &  (0.031)   \\
\addlinespace
Housing supply elasticity x Dum00t06&            &            &    0.001   &    0.002   \\
               &            &            &  (0.003)   &  (0.003)   \\
\addlinespace
Housing supply elasticity x Dum07t10&            &            &   -0.003   &   -0.004   \\
               &            &            &  (0.005)   &  (0.005)   \\
\addlinespace
House Vacancy Rate (1999) x Dum00t06&            &            &    0.063   &    0.029   \\
               &            &            &  (0.067)   &  (0.065)   \\
\addlinespace
House Vacancy Rate (1999) x Dum07t10&            &            &   -0.086   &   -0.018   \\
               &            &            &  (0.116)   &  (0.116)   \\
\addlinespace
Ratio of Renters (1999) x Dum00t06&            &            &   -0.011   &   -0.078** \\
               &            &            &  (0.032)   &  (0.040)   \\
\addlinespace
Ratio of Renters (1999) x Dum07t10&            &            &    0.039   &    0.207***\\
               &            &            &  (0.046)   &  (0.057)   \\
\addlinespace
Ratio of Bachelor Educated (1999) x Dum00t06&            &            &            &   -0.000   \\
               &            &            &            &  (0.064)   \\
\addlinespace
Ratio of Bachelor Educated (1999) x Dum07t10&            &            &            &   -0.206*  \\
               &            &            &            &  (0.107)   \\
\addlinespace
Ratio of White Race (1999) x Dum00t06&            &            &            &   -0.011   \\
               &            &            &            &  (0.024)   \\
\addlinespace
Ratio of White Race (1999) x Dum07t10&            &            &            &    0.047   \\
               &            &            &            &  (0.034)   \\
\addlinespace
Ratio of Immigration (90-00) x Dum00t06&            &            &            &    0.418***\\
               &            &            &            &  (0.149)   \\
\addlinespace
Ratio of Immigration (90-00) x Dum07t10&            &            &            &   -0.581***\\
               &            &            &            &  (0.217)   \\
\midrule
Obs            &     1580   &     1580   &     1398   &     1398   \\
Cluster SE     &     CBSA   &     CBSA   &     CBSA   &     CBSA   \\
Weight         & Ln(HU99)   & Ln(HU99)   & Ln(HU99)   & Ln(HU99)   \\
KP F-Stat (99-05, non-stack sample)       &    23.41   &    21.19   &    14.39   &    12.05   \\
MOP F-Stat (99-05, non-stack sample)  &    22.22   &    20.36   &    14.43   &    12.09   \\
CoefEqual\_Chi2  &   12.874   &    8.399   &    5.199   &    5.533   \\
CoefEqual\_PValue  &    0.000   &    0.004   &    0.023   &    0.019   \\
\bottomrule

\end{tabular}

} % end of resize box

\end{table}

==> Table_Purch/table_ResiConst.D00t06vsD07t10.PLMNJ.2SLS.tex <==
%-----------------------------------------------------------------------
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% table_ResiConst.D00t06vsD07t10.PLMNJ.2SLS
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\noindent 

\begin{table}[h!]
\centering
\caption{
\textbf{2SLS Stacked Regression of Residential Construction Employment Growth in Boom (00-06) and Bust (07-10) Periods on PLMNJ Growth (99-05)} \smallskip \newline
{\scriptsize
This table reports 2SLS regression $\triangle_{00,06} \& \triangle_{07,10} ResiConstEmpShr_{c} = \beta_{00,06} * \triangle_{99,05} Ln(PLMNJ_{c}) \times Dum_{00,06} + \beta_{07,10} * \triangle_{99,05} Ln(PLMNJ_{c}) \times Dum_{07,10} + \gamma_{00,06}* \bm{Controls_{c}} \times Dum_{00,06} + \gamma_{07,10}* \bm{Controls_{c}} \times Dum_{07,10} + \epsilon_{period, c}$. The left-hand-side dependent variable $\triangle_{00,06} \& \triangle_{07,10} ResiConstEmpShr_{c}$ is the change of the residential construction employment share in working-age population at county $c$ 00-06 and 07-10. To make the coefficient more visible in the table, the residential employment share growth is multiplied by 100. The key independent variable $\triangle_{99,05} Ln(PLMNJ_{c})$ is the growth rate of the dollar amount (07USD) of private-label mortgages (non-jumbo) at county $c$ 99-05. $Controls_{c}$ indicates control variables at county $c$ in the period start year 1999. We use the gravity model-based instrumental variable $\triangle_{99,05}\text{givNetExp}_{m}$ as the IV for $\triangle_{99,05}Ln(PLMNJ_{c})$. Regression is weighted by the natural logarithm of housing units in 1999.  For the first-stage F-test of two non-stacked samples, we report Kleibergen-Paap (2006) robust (clustered) statistics and Montiel Olea-Pflueger (2013) efficient statistics. Standard errors are clustered at the CBSA level. ***, **, and * indicate significance at the 1\%, 5\%, and 10\% levels, respectively.
\smallskip
} % end of small font size
} % end of caption
\label{table_ResiConst.D00t06vsD07t10.PLMNJ.2SLS}

\vspace{-2mm}

\resizebox{0.55\columnwidth}{!}{%
\begin{tabular}{l*{4}{c}}
\toprule
\textbf{TSLS estimates}            &\multicolumn{4}{c}{Residential Construction Employment Growth (00-06 and 07-10, An)} \\
            \cmidrule{2-5} 
            &\multicolumn{1}{c}{(1)}&\multicolumn{1}{c}{(2)}&\multicolumn{1}{c}{(3)}&\multicolumn{1}{c}{(4)}\\
            
\midrule
PLMNJ Growth (99-05, An) x Dum00t06&    0.124** &    0.144** &    0.157*  &    0.171** \\
               &  (0.056)   &  (0.062)   &  (0.084)   &  (0.087)   \\
\addlinespace
PLMNJ Growth (99-05, An) x Dum07t10&   -0.231***&   -0.232***&   -0.241** &   -0.261** \\
               &  (0.073)   &  (0.081)   &  (0.110)   &  (0.123)   \\
\addlinespace
Dum00t06       &   -0.015   &   -0.056   &   -0.092   &   -0.052   \\
               &  (0.010)   &  (0.062)   &  (0.077)   &  (0.128)   \\
\addlinespace
Dum07t10       &    0.018   &    0.274***&    0.295** &    0.095   \\
               &  (0.013)   &  (0.086)   &  (0.117)   &  (0.202)   \\
\addlinespace
Ln(Num of HH, 99) x Dum00t06&            &   -0.005***&    0.004   &    0.001   \\
               &            &  (0.001)   &  (0.010)   &  (0.011)   \\
\addlinespace
Ln(Num of HH, 99) x Dum07t10&            &    0.006***&    0.021   &    0.023   \\
               &            &  (0.002)   &  (0.014)   &  (0.015)   \\
\addlinespace
Ln(HH Income, 99) x Dum00t06&            &    0.013*  &    0.013   &    0.009   \\
               &            &  (0.007)   &  (0.008)   &  (0.013)   \\
\addlinespace
Ln(HH Income, 99) x Dum07t10&            &   -0.036***&   -0.032***&   -0.015   \\
               &            &  (0.011)   &  (0.012)   &  (0.020)   \\
\addlinespace
Ratio of Labor Force (1999) x Dum00t06&            &   -0.077***&   -0.047*  &   -0.041   \\
               &            &  (0.027)   &  (0.028)   &  (0.028)   \\
\addlinespace
Ratio of Labor Force (1999) x Dum07t10&            &    0.100** &    0.052   &    0.052   \\
               &            &  (0.043)   &  (0.041)   &  (0.042)   \\
\addlinespace
Ln(Num of HU, 99) x Dum00t06&            &            &   -0.009   &   -0.006   \\
               &            &            &  (0.010)   &  (0.011)   \\
\addlinespace
Ln(Num of HU, 99) x Dum07t10&            &            &   -0.017   &   -0.018   \\
               &            &            &  (0.014)   &  (0.015)   \\
\addlinespace
Housing supply elasticity x Dum00t06&            &            &    0.000   &    0.001   \\
               &            &            &  (0.001)   &  (0.001)   \\
\addlinespace
Housing supply elasticity x Dum07t10&            &            &   -0.001   &   -0.001   \\
               &            &            &  (0.002)   &  (0.002)   \\
\addlinespace
House Vacancy Rate (1999) x Dum00t06&            &            &    0.103***&    0.096***\\
               &            &            &  (0.037)   &  (0.037)   \\
\addlinespace
House Vacancy Rate (1999) x Dum07t10&            &            &   -0.062   &   -0.049   \\
               &            &            &  (0.058)   &  (0.058)   \\
\addlinespace
Ratio of Renters (1999) x Dum00t06&            &            &    0.016   &    0.004   \\
               &            &            &  (0.015)   &  (0.019)   \\
\addlinespace
Ratio of Renters (1999) x Dum07t10&            &            &    0.008   &    0.042   \\
               &            &            &  (0.026)   &  (0.028)   \\
\addlinespace
Ratio of Bachelor Educated (1999) x Dum00t06&            &            &            &    0.001   \\
               &            &            &            &  (0.030)   \\
\addlinespace
Ratio of Bachelor Educated (1999) x Dum07t10&            &            &            &   -0.055   \\
               &            &            &            &  (0.051)   \\
\addlinespace
Ratio of White Race (1999) x Dum00t06&            &            &            &    0.003   \\
               &            &            &            &  (0.012)   \\
\addlinespace
Ratio of White Race (1999) x Dum07t10&            &            &            &    0.014   \\
               &            &            &            &  (0.015)   \\
\addlinespace
Ratio of Immigration (90-00) x Dum00t06&            &            &            &    0.104** \\
               &            &            &            &  (0.050)   \\
\addlinespace
Ratio of Immigration (90-00) x Dum07t10&            &            &            &   -0.076   \\
               &            &            &            &  (0.085)   \\
\midrule
Obs            &     1534   &     1534   &     1355   &     1355   \\
Cluster SE     &     CBSA   &     CBSA   &     CBSA   &     CBSA   \\
Weight         & Ln(HU99)   & Ln(HU99)   & Ln(HU99)   & Ln(HU99)   \\
KP F-Stat (99-05, non-stack sample)       &    23.24   &    21.20   &    13.90   &    11.75   \\
MOP F-Stat (99-05, non-stack sample)  &    22.16   &    20.45   &    13.93   &    11.78   \\
CoefEqual\_Chi2  & 8.448   &    7.717   &    4.651   &    4.559   \\
CoefEqual\_PValue &    0.004   &    0.005   &    0.031   &    0.033   \\\\
\bottomrule

\end{tabular}

} % end of resize box

\end{table}

==> Table_Purch/table_Tradable.D00t06vsD07t10.PLMNJ.2SLS.tex <==
%-----------------------------------------------------------------------
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% table_Tradable.D00t06vsD07t10.PLMNJ.2SLS
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\noindent 

\begin{table}[h!]
\centering
\caption{
\textbf{2SLS Stacked Regression of Tradable Employment Growth in Boom (00-06) and Bust (07-10) Periods on PLMNJ Growth (99-05)} \smallskip \newline
{\scriptsize
This table reports 2SLS regression $\triangle_{00,06} \& \triangle_{07,10} TradableEmpShr_{c} = \beta_{00,06} * \triangle_{99,05} Ln(PLMNJ_{c}) \times Dum_{00,06} + \beta_{07,10} * \triangle_{99,05} Ln(PLMNJ_{c}) \times Dum_{07,10} + \gamma_{00,06}* \bm{Controls_{c}} \times Dum_{00,06} + \gamma_{07,10}* \bm{Controls_{c}} \times Dum_{07,10} + \epsilon_{period, c}$. The left-hand-side dependent variable $\triangle_{00,06} \& \triangle_{07,10} TradableEmpShr_{c}$ is the change of the Tradable employment share in working-age population at county $c$ 00-06 and 07-10. The key independent variable $\triangle_{99,05} Ln(PLMNJ_{c})$ is the growth rate of the dollar amount (07USD) of private-label mortgages (non-jumbo) at county $c$ 99-05. $Controls_{c}$ indicates control variables at county $c$ in the period start year 1999. We use the gravity model-based instrumental variable $\triangle_{99,05}\text{givNetExp}_{m}$ as the IV for $\triangle_{99,05}Ln(PLMNJ_{c})$. Regression is weighted by the natural logarithm of housing units in 1999.  For the first-stage F-test of two non-stacked samples, we report Kleibergen-Paap (2006) robust (clustered) statistics and Montiel Olea-Pflueger (2013) efficient statistics. Standard errors are clustered at the CBSA level. ***, **, and * indicate significance at the 1\%, 5\%, and 10\% levels, respectively.
\smallskip
} % end of small font size
} % end of caption
\label{table_Tradable.D00t06vsD07t10.PLMNJ.2SLS}

\vspace{-2mm}

\resizebox{0.55\columnwidth}{!}{%
\begin{tabular}{l*{4}{c}}
\toprule
\textbf{TSLS estimates}            &\multicolumn{4}{c}{Tradable Employment Growth (00-06 and 07-10, An)} \\
            \cmidrule{2-5} 
            &\multicolumn{1}{c}{(1)}&\multicolumn{1}{c}{(2)}&\multicolumn{1}{c}{(3)}&\multicolumn{1}{c}{(4)}\\
            
\midrule
PLMNJ Growth (07USD, 99-05, An) x Dum00t06&    0.061***&    0.063***&    0.066***&    0.072***\\
               &  (0.016)   &  (0.016)   &  (0.020)   &  (0.023)   \\
\addlinespace
PLMNJ Growth (07USD, 99-05, An) x Dum07t10&    0.057***&    0.061***&    0.070***&    0.078***\\
               &  (0.014)   &  (0.015)   &  (0.023)   &  (0.028)   \\
\addlinespace
Dum00t06       &   -0.013***&   -0.008   &   -0.018   &    0.064** \\
               &  (0.003)   &  (0.014)   &  (0.018)   &  (0.032)   \\
\addlinespace
Dum07t10       &   -0.013***&   -0.001   &   -0.021   &    0.082** \\
               &  (0.002)   &  (0.016)   &  (0.021)   &  (0.033)   \\
\addlinespace
Ln(Num of HH, 99) x Dum00t06&            &   -0.000** &    0.005   &    0.006   \\
               &            &  (0.000)   &  (0.004)   &  (0.005)   \\
\addlinespace
Ln(Num of HH, 99) x Dum07t10&            &   -0.000*  &   -0.002   &   -0.000   \\
               &            &  (0.000)   &  (0.003)   &  (0.003)   \\
\addlinespace
Ln(HH Income, 99) x Dum00t06&            &   -0.000   &    0.001   &   -0.006*  \\
               &            &  (0.002)   &  (0.002)   &  (0.003)   \\
\addlinespace
Ln(HH Income, 99) x Dum07t10&            &   -0.000   &    0.002   &   -0.008** \\
               &            &  (0.002)   &  (0.002)   &  (0.003)   \\
\addlinespace
Ratio of Labor Force (1999) x Dum00t06&            &    0.003   &   -0.006   &   -0.011   \\
               &            &  (0.007)   &  (0.008)   &  (0.009)   \\
\addlinespace
Ratio of Labor Force (1999) x Dum07t10&            &   -0.007   &   -0.011   &   -0.015   \\
               &            &  (0.007)   &  (0.009)   &  (0.011)   \\
\addlinespace
Ln(Num of HU, 99) x Dum00t06&            &            &   -0.005   &   -0.007   \\
               &            &            &  (0.004)   &  (0.005)   \\
\addlinespace
Ln(Num of HU, 99) x Dum07t10&            &            &    0.001   &   -0.001   \\
               &            &            &  (0.003)   &  (0.003)   \\
\addlinespace
Housing supply elasticity x Dum00t06&            &            &    0.001** &    0.001** \\
               &            &            &  (0.000)   &  (0.000)   \\
\addlinespace
Housing supply elasticity x Dum07t10&            &            &    0.001   &    0.001   \\
               &            &            &  (0.000)   &  (0.000)   \\
\addlinespace
House Vacancy Rate (1999) x Dum00t06&            &            &    0.001   &   -0.001   \\
               &            &            &  (0.009)   &  (0.010)   \\
\addlinespace
House Vacancy Rate (1999) x Dum07t10&            &            &   -0.004   &   -0.007   \\
               &            &            &  (0.009)   &  (0.010)   \\
\addlinespace
Ratio of Renters (1999) x Dum00t06&            &            &    0.006   &   -0.001   \\
               &            &            &  (0.005)   &  (0.005)   \\
\addlinespace
Ratio of Renters (1999) x Dum07t10&            &            &    0.009** &   -0.002   \\
               &            &            &  (0.005)   &  (0.005)   \\
\addlinespace
Ratio of Bachelor Educated (1999) x Dum00t06&            &            &            &    0.027***\\
               &            &            &            &  (0.009)   \\
\addlinespace
Ratio of Bachelor Educated (1999) x Dum07t10&            &            &            &    0.032***\\
               &            &            &            &  (0.009)   \\
\addlinespace
Ratio of White Race (1999) x Dum00t06&            &            &            &   -0.001   \\
               &            &            &            &  (0.003)   \\
\addlinespace
Ratio of White Race (1999) x Dum07t10&            &            &            &   -0.002   \\
               &            &            &            &  (0.003)   \\
\addlinespace
Ratio of Immigration (90-00) x Dum00t06&            &            &            &    0.001   \\
               &            &            &            &  (0.016)   \\
\addlinespace
Ratio of Immigration (90-00) x Dum07t10&            &            &            &    0.011   \\
               &            &            &            &  (0.017)   \\
\midrule
Obs            &     1584   &     1584   &     1402   &     1402   \\
Cluster SE     &     CBSA   &     CBSA   &     CBSA   &     CBSA   \\
Weight         & Ln(HU99)   & Ln(HU99)   & Ln(HU99)   & Ln(HU99)   \\
KP F-Stat (99-05, non-stack sample)       &    23.43   &    21.04   &    13.97   &    11.74   \\
MOP F-Stat (99-05, non-stack sample)  &    22.30   &    20.29   &    14.03   &    11.80   \\
CoefEqual\_Chi2  &    0.051   &    0.010   &    0.041   &    0.090   \\
CoefEqual\_PValue  &    0.822   &    0.920   &    0.840   &    0.764   \\
\bottomrule

\end{tabular}

} % end of resize box

\end{table}

==> Table_Purch/table_Tradable.D00t06vsD07t10.PLMNJ.2SLS.wide.tex <==
%-----------------------------------------------------------------------
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% table_Tradable.D00t06vsD07t10.PLMNJ.2SLS.wide
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\noindent 

\begin{table}[h!]
\centering
\caption{
\textbf{2SLS Stacked Regression of Tradable Employment Growth in Boom (00-06) and Bust (07-10) Periods on PLMNJ Growth (99-05)} \smallskip \newline
{\scriptsize
This table reports 2SLS regression $\triangle_{00,06} \& \triangle_{07,10} TradableEmpShr_{c} = \beta_{00,06} * \triangle_{99,05} Ln(PLMNJ_{c}) \times Dum_{00,06} + \beta_{07,10} * \triangle_{99,05} Ln(PLMNJ_{c}) \times Dum_{07,10} + \gamma_{00,06}* \bm{Controls_{c}} \times Dum_{00,06} + \gamma_{07,10}* \bm{Controls_{c}} \times Dum_{07,10} + \epsilon_{period, c}$. The left-hand-side dependent variable $\triangle_{00,06} \& \triangle_{07,10} TradableEmpShr_{c}$ is the change of the Tradable employment share in working-age population at county $c$ 00-06 and 07-10. The key independent variable $\triangle_{99,05} Ln(PLMNJ_{c})$ is the growth rate of the dollar amount (07USD) of private-label mortgages (non-jumbo) at county $c$ 99-05. $Controls_{c}$ indicates control variables at county $c$ in the period start year 1999. We use the gravity model-based instrumental variable $\triangle_{99,05}\text{givNetExp}_{m}$ as the IV for $\triangle_{99,05}Ln(PLMNJ_{c})$. Regression is weighted by the natural logarithm of housing units in 1999.  For the first-stage F-test of two non-stacked samples, we report Kleibergen-Paap (2006) robust (clustered) statistics and Montiel Olea-Pflueger (2013) efficient statistics. Standard errors are clustered at the CBSA level. ***, **, and * indicate significance at the 1\%, 5\%, and 10\% levels, respectively.
\smallskip
} % end of small font size
} % end of caption
\label{table_Tradable.D00t06vsD07t10.PLMNJ.2SLS.wide}

\vspace{-2mm}

\resizebox{\columnwidth}{!}{%
\begin{tabular}{l*{8}{c}}
\toprule
\textbf{TSLS estimates}            &\multicolumn{8}{c}{Tradable Employment Growth (00-06 and 07-10, An)} \\
            \cmidrule{2-9} 
            &\multicolumn{2}{c}{(1)}&\multicolumn{2}{c}{(2)}&\multicolumn{2}{c}{(3)}&\multicolumn{2}{c}{(4)}\\
            
\midrule
PLMNJ Growth (07USD, 99-05, An) x Dum00t06&    0.061***&  (0.016)&    0.063***&  (0.016)&    0.066***&  (0.020)&    0.072***&  (0.023)\\
PLMNJ Growth (07USD, 99-05, An) x Dum07t10&    0.057***&  (0.014)&    0.061***&  (0.015)&    0.070***&  (0.023)&    0.078***&  (0.028)\\
Dum00t06       &   -0.013***&  (0.003)&   -0.008   &  (0.014)&   -0.018   &  (0.018)&    0.064** &  (0.032)\\
Dum07t10       &   -0.013***&  (0.002)&   -0.001   &  (0.016)&   -0.021   &  (0.021)&    0.082** &  (0.033)\\
Ln(Num of HH, 99) x Dum00t06&            &         &   -0.000** &  (0.000)&    0.005   &  (0.004)&    0.006   &  (0.005)\\
Ln(Num of HH, 99) x Dum07t10&            &         &   -0.000*  &  (0.000)&   -0.002   &  (0.003)&   -0.000   &  (0.003)\\
Ln(HH Income, 99) x Dum00t06&            &         &   -0.000   &  (0.002)&    0.001   &  (0.002)&   -0.006*  &  (0.003)\\
Ln(HH Income, 99) x Dum07t10&            &         &   -0.000   &  (0.002)&    0.002   &  (0.002)&   -0.008** &  (0.003)\\
Ratio of Labor Force (1999) x Dum00t06&            &         &    0.003   &  (0.007)&   -0.006   &  (0.008)&   -0.011   &  (0.009)\\
Ratio of Labor Force (1999) x Dum07t10&            &         &   -0.007   &  (0.007)&   -0.011   &  (0.009)&   -0.015   &  (0.011)\\
Ln(Num of HU, 99) x Dum00t06&            &         &            &         &   -0.005   &  (0.004)&   -0.007   &  (0.005)\\
Ln(Num of HU, 99) x Dum07t10&            &         &            &         &    0.001   &  (0.003)&   -0.001   &  (0.003)\\
Housing supply elasticity x Dum00t06&            &         &            &         &    0.001** &  (0.000)&    0.001** &  (0.000)\\
Housing supply elasticity x Dum07t10&            &         &            &         &    0.001   &  (0.000)&    0.001   &  (0.000)\\
House Vacancy Rate (1999) x Dum00t06&            &         &            &         &    0.001   &  (0.009)&   -0.001   &  (0.010)\\
House Vacancy Rate (1999) x Dum07t10&            &         &            &         &   -0.004   &  (0.009)&   -0.007   &  (0.010)\\
Ratio of Renters (1999) x Dum00t06&            &         &            &         &    0.006   &  (0.005)&   -0.001   &  (0.005)\\
Ratio of Renters (1999) x Dum07t10&            &         &            &         &    0.009** &  (0.005)&   -0.002   &  (0.005)\\
Ratio of Bachelor Educated (1999) x Dum00t06&            &         &            &         &            &         &    0.027***&  (0.009)\\
Ratio of Bachelor Educated (1999) x Dum07t10&            &         &            &         &            &         &    0.032***&  (0.009)\\
Ratio of White Race (1999) x Dum00t06&            &         &            &         &            &         &   -0.001   &  (0.003)\\
Ratio of White Race (1999) x Dum07t10&            &         &            &         &            &         &   -0.002   &  (0.003)\\
Ratio of Immigration (90-00) x Dum00t06&            &         &            &         &            &         &    0.001   &  (0.016)\\
Ratio of Immigration (90-00) x Dum07t10&            &         &            &         &            &         &    0.011   &  (0.017)\\
\midrule
Obs            &     1584   &         &     1584   &         &     1402   &         &     1402   &         \\
Cluster SE     &     CBSA   &         &     CBSA   &         &     CBSA   &         &     CBSA   &         \\
Weight         & Ln(HU99)   &         & Ln(HU99)   &         & Ln(HU99)   &         & Ln(HU99)   &         \\
KP F-Stat (99-05, non-stack sample)      &    23.43   &         &    21.04   &         &    13.97   &         &    11.74   &         \\
MOP F-Stat (99-05, non-stack sample)  &    22.30   &         &    20.29   &         &    14.03   &         &    11.80   &         \\
CoefEqual\_Chi2 &    0.051   &         &    0.010   &         &    0.041   &         &    0.090   &         \\
CoefEqual\_PValue &    0.822   &         &    0.920   &         &    0.840   &         &    0.764   &         \\
\bottomrule

\end{tabular}

} % end of resize box

\end{table}
